ThinkJev: One Thought, Every Budget for Calibrated Typed Decisions

Many uses of language models end in a typed decision: a choice among a closed set of options, whose probabilities code can act on. Reading those probabilities from one forward pass is fast but often wrong on decisions that take several steps, such as arithmetic, counting, and date comparison. Letting the model think first fixes most of these errors, but costs seconds per decision instead of milliseconds. To pay for thinking only where it helps, ThinkJev builds a fast and a slow system from one open hybrid-thinking model that can answer directly or after a thought. System 1 reads the model's probabilities for the option letters when it answers directly; System 2 reads the same letters after the model has thought on the same cached prompt, so escalating repeats no work and both systems give probabilities over the same options. Because the letters can be read after any number of thought tokens, one sampled thought also gives the answer under every thinking budget. Without training, ThinkJev lets System 1 answer alone only where a statistical test on labeled dev data guarantees that its accepted answers stay under a target error rate. At a 5% target, Qwen3.5-27B answers 24.5% of 8359 test decisions this way with a realized error of 3.9% (Qwen3.5-4B and 9B: 6.5% and 0.0%). For the rest, stopping each thought as soon as its answer is confident reaches 81.6% accuracy, against 82.7% for always thinking, with 72% of the thought tokens. Choosing when to think from System 1's confidence alone saves less, because the decisions System 1 is least sure of are often not the ones thinking fixes. On the public items of JevBench, an independent benchmark of typed-decision services, Qwen3.5-27B thinks on 29.4% and is not distinguishable in accuracy from the two thinking APIs listed (exploratory). Code and data generators are available at https://github.com/ding-xiaolu/ThinkJev.

==> figures/qwen3.5-27b/data.tex <==
A & Escalation (CLINC) & 210 & 290 & en & CC-BY-3.0 \\
A & Every judgments & 70 & 84 & en & unstated \\
A & Intent routing (BANKING77) & 313 & 486 & en & CC-BY-4.0 \\
A & Intent routing (CLINC) & 242 & 358 & en & CC-BY-3.0 \\
A & NLI (WANLI) & 97 & 159 & en & CC-BY-4.0 \\
A & SemIf authored & 60 & 84 & en & MIT \\
A & Typed decisions & 835 & 1165 & en & Apache-2.0 \\
\midrule
B & BIG-Bench Hard & 400 & 620 & en & MIT \\
B & GPQA Diamond & 81 & 117 & en & CC-BY-4.0 \\
B & MMLU-Pro & 475 & 715 & en & MIT \\
B & MuSR & 217 & 383 & en & CC-BY-4.0 \\
B & SuperGPQA & 428 & 652 & en & ODC-BY-1.0 \\
\midrule
C & Chess (Lichess) & 467 & 733 & en, zh & CC0-1.0 \\
C & Generated families & 1608 & 2392 & en, zh & MIT \\
C & hard200 fixture & 79 & 121 & en & MIT \\
\midrule
All & & 5582 & 8359 & & \\


==> figures/qwen3.5-27b/numbers.tex <==
\tjset{rows_test}{8359} % `rows.test`
\tjset{always_s1_accuracy}{62.2\%} % `baselines_test.always_s1_accuracy`
\tjset{always_s2_accuracy}{82.7\%} % `baselines_test.always_s2_accuracy`
\tjset{always_s2_mean_think_tokens}{1856} % `baselines_test.s2_mean_think_tokens`
\tjset{s1_wrong_s2_right}{1971} % `baselines_test.s1_wrong_s2_right`
\tjset{s1_right_s2_wrong}{260} % `baselines_test.s1_right_s2_wrong`
\tjset{s1_ece}{0.024} % `s1_readouts_test.*.ece`
\tjset{gate_test_accuracy}{81.6\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_mean_think_tokens}{1511} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_thinking_share}{81\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{anytime_test_accuracy}{81.6\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_mean_think_tokens}{1344} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_thinking_share}{72\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{s1_ltt_coverage_at_5pct}{24.5\%} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_5pct}{3.9\%} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_risk)
\tjset{block_all_rows}{8359} % `per_family_test` (rows, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s1}{62.2\%} % `per_family_test` (s1_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s2}{82.7\%} % `per_family_test` (s2_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_system}{81.6\%} % `per_family_test` (system_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_escalation}{62.4\%} % `per_family_test` (escalation_rate, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_jev_rows}{2626} % `per_family_test` (rows, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s1}{77.6\%} % `per_family_test` (s1_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s2}{80.8\%} % `per_family_test` (s2_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_system}{80.7\%} % `per_family_test` (system_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_escalation}{39.5\%} % `per_family_test` (escalation_rate, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_public_rows}{2487} % `per_family_test` (rows, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s1}{58.9\%} % `per_family_test` (s1_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s2}{78.4\%} % `per_family_test` (s2_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_system}{78.2\%} % `per_family_test` (system_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_escalation}{67.6\%} % `per_family_test` (escalation_rate, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_weak_rows}{3246} % `per_family_test` (rows, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s1}{52.3\%} % `per_family_test` (s1_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s2}{87.5\%} % `per_family_test` (s2_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_system}{84.9\%} % `per_family_test` (system_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_escalation}{77.1\%} % `per_family_test` (escalation_rate, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{oracle_accuracy}{85.8\%} % `baselines_test.oracle_best_accuracy`
\tjset{s2_closed_naturally}{81.0\%} % `baselines_test.s2_closed_naturally_rate`
\tjset{disagree_total}{2231} % `baselines_test.s1_wrong_s2_right` + `s1_right_s2_wrong`
\tjset{h2_accuracy}{81.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{h2_gap}{1.1} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, always-S2 accuracy minus test_accuracy, in points)
\tjset{h2_escalation}{62.4\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{s1_raw_accuracy}{62.2\%} % `s1_readouts_test.raw.accuracy`
\tjset{s1_raw_ece}{0.027} % `s1_readouts_test.raw.ece`
\tjset{s1_rotation_accuracy}{64.2\%} % `s1_readouts_test.rotation.accuracy`
\tjset{s1_rotation_ece}{0.024} % `s1_readouts_test.rotation.ece`
\tjset{s1_ece_uncalibrated}{0.115} % `s1_readouts_test.rotation.ece_t1`
\tjset{s1_prior_accuracy}{63.6\%} % `s1_readouts_test.rotation_batch_prior.accuracy`
\tjset{s1_prior_ece}{0.086} % `s1_readouts_test.rotation_batch_prior.ece`
\tjset{s1_order_flip_rate}{37.5\%} % `order_flip_rate_test.all`
\tjset{temp_s1}{1.68} % `s1_readouts_test.rotation.temperature`
\tjset{s1_ltt_coverage_at_1pct}{0.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_1pct}{--} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_risk)
\tjset{s1_ltt_interval_at_1pct}{} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_2pct}{3.5\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_2pct}{0.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_risk)
\tjset{s1_ltt_interval_at_2pct}{[0.0, 1.2]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_interval_at_5pct}{[3.1, 4.8]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.05, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_10pct}{38.3\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_10pct}{9.9\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_risk)
\tjset{s1_ltt_interval_at_10pct}{[8.9, 11.0]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_targets_certified}{3} % `s1_readouts_test.rotation.coverage_at_risk` (targets with ltt_test_coverage > 0)
\tjset{anytime_acc_t0}{61.8\%} % `anytime_test.per_checkpoint` (t = 0, accuracy)
\tjset{anytime_ece_t0}{0.035} % `anytime_test.per_checkpoint` (t = 0, ece)
\tjset{anytime_tokens_t0}{0} % `anytime_test.per_checkpoint` (t = 0, mean_think_tokens)
\tjset{anytime_acc_t128}{61.8\%} % `anytime_test.per_checkpoint` (t = 128, accuracy)
\tjset{anytime_ece_t128}{0.029} % `anytime_test.per_checkpoint` (t = 128, ece)
\tjset{anytime_tokens_t128}{128} % `anytime_test.per_checkpoint` (t = 128, mean_think_tokens)
\tjset{anytime_acc_t256}{62.7\%} % `anytime_test.per_checkpoint` (t = 256, accuracy)
\tjset{anytime_ece_t256}{0.030} % `anytime_test.per_checkpoint` (t = 256, ece)
\tjset{anytime_tokens_t256}{256} % `anytime_test.per_checkpoint` (t = 256, mean_think_tokens)
\tjset{anytime_acc_t512}{68.9\%} % `anytime_test.per_checkpoint` (t = 512, accuracy)
\tjset{anytime_ece_t512}{0.017} % `anytime_test.per_checkpoint` (t = 512, ece)
\tjset{anytime_tokens_t512}{506} % `anytime_test.per_checkpoint` (t = 512, mean_think_tokens)
\tjset{anytime_acc_t1024}{77.4\%} % `anytime_test.per_checkpoint` (t = 1024, accuracy)
\tjset{anytime_ece_t1024}{0.029} % `anytime_test.per_checkpoint` (t = 1024, ece)
\tjset{anytime_tokens_t1024}{879} % `anytime_test.per_checkpoint` (t = 1024, mean_think_tokens)
\tjset{anytime_acc_t2048}{81.4\%} % `anytime_test.per_checkpoint` (t = 2048, accuracy)
\tjset{anytime_ece_t2048}{0.025} % `anytime_test.per_checkpoint` (t = 2048, ece)
\tjset{anytime_tokens_t2048}{1317} % `anytime_test.per_checkpoint` (t = 2048, mean_think_tokens)
\tjset{anytime_acc_full}{82.7\%} % `anytime_test.full_thought.accuracy`
\tjset{anytime_ece_full}{0.036} % `anytime_test.full_thought.ece`
\tjset{temp_t0}{1.61} % `anytime_test.per_checkpoint` (t = 0, temperature)
\tjset{temp_t128}{1.83} % `anytime_test.per_checkpoint` (t = 128, temperature)
\tjset{temp_t256}{1.91} % `anytime_test.per_checkpoint` (t = 256, temperature)
\tjset{temp_t512}{2.21} % `anytime_test.per_checkpoint` (t = 512, temperature)
\tjset{temp_t1024}{3.06} % `anytime_test.per_checkpoint` (t = 1024, temperature)
\tjset{temp_t2048}{3.65} % `anytime_test.per_checkpoint` (t = 2048, temperature)
\tjset{temp_full}{4.07} % `anytime_test.full_thought.temperature`
\tjset{gate_eps0_accuracy}{82.7\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_accuracy)
\tjset{gate_eps0_escalation}{89.5\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, 1 - test_coverage)
\tjset{gate_eps0_share}{97\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps0_accuracy}{82.7\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_accuracy)
\tjset{anytime_eps0_share}{97\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps1_accuracy}{81.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{gate_eps1_escalation}{62.4\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{gate_eps1_share}{81\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps1_accuracy}{81.6\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_accuracy)
\tjset{anytime_eps1_share}{72\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps2_accuracy}{80.5\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_accuracy)
\tjset{gate_eps2_escalation}{53.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, 1 - test_coverage)
\tjset{gate_eps2_share}{72\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps2_accuracy}{80.6\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_accuracy)
\tjset{anytime_eps2_share}{63\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{stop_s1}{35.5\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered by S1
\tjset{stop_checkpoint}{25.5\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered at a checkpoint before the full thought
\tjset{stop_full}{39.0\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered after the full thought
\tjset{stop_checkpoint_of_escalated}{39.6\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of escalated rows that stop at a checkpoint
\tjset{lang_en_rows}{1445} % `per_family_test` (rows, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s1}{54.1\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s2}{99.5\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_system}{96.0\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_escalation}{71.7\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'en')
\tjset{lang_zh_rows}{947} % `per_family_test` (rows, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s1}{54.8\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s2}{99.7\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_system}{96.7\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_escalation}{74.8\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'zh')
\tjset{combined_eps0_accuracy}{82.7\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_accuracy)
\tjset{combined_eps0_escalation}{88.5\%} % `dev_selected_operating_points` (combined, tolerance 0.0, 1 - test_coverage)
\tjset{combined_eps0_share}{96\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps1_accuracy}{81.4\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_accuracy)
\tjset{combined_eps1_escalation}{60.1\%} % `dev_selected_operating_points` (combined, tolerance 0.01, 1 - test_coverage)
\tjset{combined_eps1_share}{79\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps2_accuracy}{80.5\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_accuracy)
\tjset{combined_eps2_escalation}{52.1\%} % `dev_selected_operating_points` (combined, tolerance 0.02, 1 - test_coverage)
\tjset{combined_eps2_share}{71\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_weight_confidence_rot}{1.355} % `combined_fit.standardized_weights.confidence_rot`
\tjset{combined_weight_router_zero_shot}{0.076} % `combined_fit.standardized_weights.router_zero_shot`
\tjset{auroc_confidence}{0.805} % `auroc_s1_correct_test.confidence`
\tjset{auroc_confidence_rot}{0.803} % `auroc_s1_correct_test.confidence_rot`
\tjset{auroc_probe}{0.770} % `auroc_s1_correct_test.probe`
\tjset{auroc_router_probe}{0.757} % `auroc_s1_correct_test.router_probe`
\tjset{auroc_router_zero_shot}{0.705} % `auroc_s1_correct_test.router_zero_shot`
\tjset{auroc_router_supervised}{0.695} % `auroc_s1_correct_test.router_supervised`
\tjset{auroc_combined}{0.803} % `auroc_s1_correct_test.combined`
\tjset{area_confidence}{0.449} % `normalized_area_test.area.confidence`
\tjset{area_confidence_rot}{0.436} % `normalized_area_test.area.confidence_rot`
\tjset{area_probe}{0.397} % `normalized_area_test.area.probe`
\tjset{area_router_probe}{0.396} % `normalized_area_test.area.router_probe`
\tjset{area_router_zero_shot}{0.491} % `normalized_area_test.area.router_zero_shot`
\tjset{area_router_supervised}{0.315} % `normalized_area_test.area.router_supervised`
\tjset{area_combined}{0.449} % `normalized_area_test.area.combined`
\tjset{area_diff_confidence}{$-$0.013} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_confidence}{[$-$0.035, +0.008]} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, ci95)
\tjset{area_diff_probe}{+0.040} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_probe}{[+0.012, +0.065]} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_probe}{+0.040} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_probe}{[+0.014, +0.068]} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_zero_shot}{$-$0.054} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_zero_shot}{[$-$0.080, $-$0.027]} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_supervised}{+0.121} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_supervised}{[+0.092, +0.152]} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, ci95)
\tjset{area_diff_combined}{$-$0.013} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_combined}{[$-$0.014, $-$0.011]} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, ci95)
\tjset{disagree_jev_fix}{183} % `disagreement_test.by_source` (summed over block 'jev', s1_wrong_s2_right)
\tjset{disagree_jev_break}{99} % `disagreement_test.by_source` (summed over block 'jev', s1_right_s2_wrong)
\tjset{disagree_public_fix}{576} % `disagreement_test.by_source` (summed over block 'public', s1_wrong_s2_right)
\tjset{disagree_public_break}{91} % `disagreement_test.by_source` (summed over block 'public', s1_right_s2_wrong)
\tjset{disagree_weak_fix}{1212} % `disagreement_test.by_source` (summed over block 'weak', s1_wrong_s2_right)
\tjset{disagree_weak_break}{70} % `disagreement_test.by_source` (summed over block 'weak', s1_right_s2_wrong)
\tjset{grp_datecomparison_rows}{293} % `per_family_test` (rows, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s1}{35.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s2}{99.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_system}{99.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_escalation}{99.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date comparison')
\tjset{grp_arithmetic_rows}{288} % `per_family_test` (rows, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s1}{37.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_escalation}{99.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Arithmetic')
\tjset{grp_chess_rows}{733} % `per_family_test` (rows, row-weighted over group 'Chess')
\tjset{grp_chess_s1}{40.4\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_s2}{45.8\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_system}{45.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_escalation}{97.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chess')
\tjset{grp_logicgrid_rows}{272} % `per_family_test` (rows, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s1}{47.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s2}{99.3\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_system}{98.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_escalation}{89.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Logic grid')
\tjset{grp_datedeadlines_rows}{27} % `per_family_test` (rows, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s1}{48.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_system}{81.5\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_escalation}{44.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date deadlines')
\tjset{grp_graphpaths_rows}{313} % `per_family_test` (rows, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s1}{49.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s2}{98.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_system}{93.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_escalation}{72.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'Graph paths')
\tjset{grp_chainedrules_rows}{298} % `per_family_test` (rows, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s1}{53.7\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_system}{84.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_escalation}{48.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chained rules')
\tjset{grp_counting_rows}{345} % `per_family_test` (rows, row-weighted over group 'Counting')
\tjset{grp_counting_s1}{65.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_system}{98.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_escalation}{63.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'Counting')
\tjset{grp_scheduling_rows}{301} % `per_family_test` (rows, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s1}{66.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_escalation}{66.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Scheduling')
\tjset{grp_stackednegation_rows}{315} % `per_family_test` (rows, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s1}{78.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s2}{99.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_system}{97.5\%} % `per_family_test` (system_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_escalation}{47.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'Stacked negation')
\tjset{grp_multihopruleshard200_rows}{31} % `per_family_test` (rows, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s1}{90.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_escalation}{25.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_doublenegationhard200_rows}{30} % `per_family_test` (rows, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s1}{100.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_escalation}{10.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Double negation (hard200)')
\tjset{grp_escalationclinc_rows}{290} % `per_family_test` (rows, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s1}{60.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s2}{72.4\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_system}{71.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_escalation}{43.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_typeddecisions_rows}{1165} % `per_family_test` (rows, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s1}{71.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s2}{73.3\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_system}{73.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_escalation}{61.5\%} % `per_family_test` (escalation_rate, row-weighted over group 'Typed decisions')
\tjset{grp_nliwanli_rows}{159} % `per_family_test` (rows, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s1}{75.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s2}{81.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_system}{79.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_escalation}{32.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'NLI (WANLI)')
\tjset{grp_intentroutingbanking77_rows}{486} % `per_family_test` (rows, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s1}{85.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s2}{86.4\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_system}{86.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_escalation}{18.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_semifauthored_rows}{84} % `per_family_test` (rows, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s1}{92.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s2}{94.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_system}{95.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_escalation}{10.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'SemIf authored')
\tjset{grp_everyjudgments_rows}{84} % `per_family_test` (rows, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s1}{95.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s2}{95.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_system}{95.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_escalation}{7.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'Every judgments')
\tjset{grp_intentroutingclinc_rows}{358} % `per_family_test` (rows, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s1}{95.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s2}{97.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_system}{97.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_escalation}{9.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_supergpqa_rows}{652} % `per_family_test` (rows, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s1}{47.7\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s2}{62.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_system}{62.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_escalation}{83.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'SuperGPQA')
\tjset{grp_mmlupro_rows}{715} % `per_family_test` (rows, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s1}{56.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s2}{82.9\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_system}{82.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_escalation}{71.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'MMLU-Pro')
\tjset{grp_gpqadiamond_rows}{117} % `per_family_test` (rows, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s1}{60.7\%} % `per_family_test` (s1_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s2}{85.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_system}{85.5\%} % `per_family_test` (system_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_escalation}{78.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'GPQA Diamond')
\tjset{grp_musr_rows}{383} % `per_family_test` (rows, row-weighted over group 'MuSR')
\tjset{grp_musr_s1}{62.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_s2}{68.9\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_system}{68.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_escalation}{51.2\%} % `per_family_test` (escalation_rate, row-weighted over group 'MuSR')
\tjset{grp_bigbenchhard_rows}{620} % `per_family_test` (rows, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s1}{70.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s2}{94.8\%} % `per_family_test` (s2_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_system}{94.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_escalation}{53.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'BIG-Bench Hard')
\tjset{difficulty_families}{9} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty computed per family)
\tjset{difficulty_rising}{7} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty > 0)
\tjset{weak_d1_rows}{767} % `per_family_test` (rows, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_escalation}{60.0\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s1}{66.6\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s2}{92.3\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d2_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_escalation}{71.7\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s1}{58.9\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s2}{86.5\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d3_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_escalation}{89.0\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s1}{39.8\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s2}{86.0\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d4_rows}{776} % `per_family_test` (rows, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_escalation}{94.1\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s1}{39.3\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s2}{83.2\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 4)
\tjset{jb_s1_correct}{207} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s1` (correct)
\tjset{jb_s1_acc}{89.6\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s1` (accuracy)
\tjset{jb_s1_hard_correct}{90} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s1` (by_tier.hard.correct)
\tjset{jb_s1_hard_acc}{81.1\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s1` (by_tier.hard.accuracy)
\tjset{jb_s1_ece}{0.047} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s1` (ece)
\tjset{jb_s1_think}{0} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s1` (mean_think_tokens)
\tjset{jb_s1_escalation}{0.0\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s1` (escalation_rate)
\tjset{jb_s1_vs_jev1130_all_ours}{12} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.jev-1.13.0.all` (ours_only)
\tjset{jb_s1_vs_jev1130_all_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.jev-1.13.0.all` (theirs_only)
\tjset{jb_s1_vs_jev1130_all_p}{$p = 0.143$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.jev-1.13.0.all` (p_value)
\tjset{jb_s1_vs_jev1130_hard_ours}{12} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.jev-1.13.0.hard` (ours_only)
\tjset{jb_s1_vs_jev1130_hard_theirs}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s1_vs_jev1130_hard_p}{$p = 0.035$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.jev-1.13.0.hard` (p_value)
\tjset{jb_s1_vs_openjevthinking_all_ours}{13} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.openjev-thinking.all` (ours_only)
\tjset{jb_s1_vs_openjevthinking_all_theirs}{11} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.openjev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_all_p}{$p = 0.839$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.openjev-thinking.all` (p_value)
\tjset{jb_s1_vs_openjevthinking_hard_ours}{13} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.openjev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_openjevthinking_hard_theirs}{8} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.openjev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_hard_p}{$p = 0.383$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.openjev-thinking.hard` (p_value)
\tjset{jb_s1_vs_djevthinking_all_ours}{21} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.djev-thinking.all` (ours_only)
\tjset{jb_s1_vs_djevthinking_all_theirs}{16} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.djev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_djevthinking_all_p}{$p = 0.511$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.djev-thinking.all` (p_value)
\tjset{jb_s1_vs_djevthinking_hard_ours}{18} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.djev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_djevthinking_hard_theirs}{13} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.djev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_djevthinking_hard_p}{$p = 0.473$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.djev-thinking.hard` (p_value)
\tjset{jb_s1_vs_semifqwen354b_all_ours}{26} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_all_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s1_vs_semifqwen354b_hard_ours}{25} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_hard_theirs}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s1_vs_reflex27b_all_ours}{12} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.reflex-27b.all` (ours_only)
\tjset{jb_s1_vs_reflex27b_all_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.reflex-27b.all` (theirs_only)
\tjset{jb_s1_vs_reflex27b_all_p}{$p = 0.238$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.reflex-27b.all` (p_value)
\tjset{jb_s1_vs_reflex27b_hard_ours}{11} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.reflex-27b.hard` (ours_only)
\tjset{jb_s1_vs_reflex27b_hard_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.reflex-27b.hard` (theirs_only)
\tjset{jb_s1_vs_reflex27b_hard_p}{$p = 0.210$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.reflex-27b.hard` (p_value)
\tjset{jb_s1_vs_deepseekflash_all_ours}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.deepseek-flash.all` (ours_only)
\tjset{jb_s1_vs_deepseekflash_all_theirs}{22} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.deepseek-flash.all` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.deepseek-flash.all` (p_value)
\tjset{jb_s1_vs_deepseekflash_hard_ours}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.deepseek-flash.hard` (ours_only)
\tjset{jb_s1_vs_deepseekflash_hard_theirs}{19} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.deepseek-flash.hard` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.deepseek-flash.hard` (p_value)
\tjset{jb_s1_vs_gpt56luna_all_ours}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s1_vs_gpt56luna_all_theirs}{21} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (p_value)
\tjset{jb_s1_vs_gpt56luna_hard_ours}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s1_vs_gpt56luna_hard_theirs}{19} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (p_value)
\tjset{jb_s2_correct}{226} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s2` (correct)
\tjset{jb_s2_acc}{97.8\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s2` (accuracy)
\tjset{jb_s2_hard_correct}{106} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s2` (by_tier.hard.correct)
\tjset{jb_s2_hard_acc}{95.5\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s2` (by_tier.hard.accuracy)
\tjset{jb_s2_ece}{0.068} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s2` (ece)
\tjset{jb_s2_think}{1307} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s2` (mean_think_tokens)
\tjset{jb_s2_escalation}{100.0\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.s2` (escalation_rate)
\tjset{jb_s2_vs_jev1130_all_ours}{28} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.jev-1.13.0.all` (ours_only)
\tjset{jb_s2_vs_jev1130_all_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.jev-1.13.0.all` (theirs_only)
\tjset{jb_s2_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.jev-1.13.0.all` (p_value)
\tjset{jb_s2_vs_jev1130_hard_ours}{27} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.jev-1.13.0.hard` (ours_only)
\tjset{jb_s2_vs_jev1130_hard_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s2_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.jev-1.13.0.hard` (p_value)
\tjset{jb_s2_vs_openjevthinking_all_ours}{22} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.openjev-thinking.all` (ours_only)
\tjset{jb_s2_vs_openjevthinking_all_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.openjev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.openjev-thinking.all` (p_value)
\tjset{jb_s2_vs_openjevthinking_hard_ours}{22} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.openjev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_openjevthinking_hard_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.openjev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.openjev-thinking.hard` (p_value)
\tjset{jb_s2_vs_djevthinking_all_ours}{28} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.djev-thinking.all` (ours_only)
\tjset{jb_s2_vs_djevthinking_all_theirs}{4} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.djev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_djevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.djev-thinking.all` (p_value)
\tjset{jb_s2_vs_djevthinking_hard_ours}{25} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.djev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_djevthinking_hard_theirs}{4} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.djev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_djevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.djev-thinking.hard` (p_value)
\tjset{jb_s2_vs_semifqwen354b_all_ours}{40} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_all_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s2_vs_semifqwen354b_hard_ours}{39} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_hard_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s2_vs_reflex27b_all_ours}{27} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.reflex-27b.all` (ours_only)
\tjset{jb_s2_vs_reflex27b_all_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.reflex-27b.all` (theirs_only)
\tjset{jb_s2_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.reflex-27b.all` (p_value)
\tjset{jb_s2_vs_reflex27b_hard_ours}{24} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.reflex-27b.hard` (ours_only)
\tjset{jb_s2_vs_reflex27b_hard_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.reflex-27b.hard` (theirs_only)
\tjset{jb_s2_vs_reflex27b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.reflex-27b.hard` (p_value)
\tjset{jb_s2_vs_deepseekflash_all_ours}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.deepseek-flash.all` (ours_only)
\tjset{jb_s2_vs_deepseekflash_all_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.deepseek-flash.all` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_all_p}{$p = 1.000$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.deepseek-flash.all` (p_value)
\tjset{jb_s2_vs_deepseekflash_hard_ours}{4} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.deepseek-flash.hard` (ours_only)
\tjset{jb_s2_vs_deepseekflash_hard_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.deepseek-flash.hard` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_hard_p}{$p = 1.000$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.deepseek-flash.hard` (p_value)
\tjset{jb_s2_vs_gpt56luna_all_ours}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s2_vs_gpt56luna_all_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_all_p}{$p = 1.000$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (p_value)
\tjset{jb_s2_vs_gpt56luna_hard_ours}{4} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s2_vs_gpt56luna_hard_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_hard_p}{$p = 1.000$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (p_value)
\tjset{jb_gate_correct}{224} % `jevbench-qwen3.5-27b-report-v2.json` `policies.gate` (correct)
\tjset{jb_gate_acc}{97.0\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.gate` (accuracy)
\tjset{jb_gate_hard_correct}{104} % `jevbench-qwen3.5-27b-report-v2.json` `policies.gate` (by_tier.hard.correct)
\tjset{jb_gate_hard_acc}{93.7\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.gate` (by_tier.hard.accuracy)
\tjset{jb_gate_ece}{0.039} % `jevbench-qwen3.5-27b-report-v2.json` `policies.gate` (ece)
\tjset{jb_gate_think}{742} % `jevbench-qwen3.5-27b-report-v2.json` `policies.gate` (mean_think_tokens)
\tjset{jb_gate_escalation}{29.4\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.gate` (escalation_rate)
\tjset{jb_gate_vs_jev1130_all_ours}{26} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.jev-1.13.0.all` (ours_only)
\tjset{jb_gate_vs_jev1130_all_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.jev-1.13.0.all` (theirs_only)
\tjset{jb_gate_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.jev-1.13.0.all` (p_value)
\tjset{jb_gate_vs_jev1130_hard_ours}{25} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.jev-1.13.0.hard` (ours_only)
\tjset{jb_gate_vs_jev1130_hard_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.jev-1.13.0.hard` (theirs_only)
\tjset{jb_gate_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.jev-1.13.0.hard` (p_value)
\tjset{jb_gate_vs_openjevthinking_all_ours}{20} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.openjev-thinking.all` (ours_only)
\tjset{jb_gate_vs_openjevthinking_all_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.openjev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.openjev-thinking.all` (p_value)
\tjset{jb_gate_vs_openjevthinking_hard_ours}{20} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.openjev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_openjevthinking_hard_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.openjev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.openjev-thinking.hard` (p_value)
\tjset{jb_gate_vs_djevthinking_all_ours}{27} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.djev-thinking.all` (ours_only)
\tjset{jb_gate_vs_djevthinking_all_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.djev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_djevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.djev-thinking.all` (p_value)
\tjset{jb_gate_vs_djevthinking_hard_ours}{24} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.djev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_djevthinking_hard_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.djev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_djevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.djev-thinking.hard` (p_value)
\tjset{jb_gate_vs_semifqwen354b_all_ours}{38} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_all_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_gate_vs_semifqwen354b_hard_ours}{37} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_hard_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_gate_vs_reflex27b_all_ours}{25} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.reflex-27b.all` (ours_only)
\tjset{jb_gate_vs_reflex27b_all_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.reflex-27b.all` (theirs_only)
\tjset{jb_gate_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.reflex-27b.all` (p_value)
\tjset{jb_gate_vs_reflex27b_hard_ours}{22} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.reflex-27b.hard` (ours_only)
\tjset{jb_gate_vs_reflex27b_hard_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.reflex-27b.hard` (theirs_only)
\tjset{jb_gate_vs_reflex27b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.reflex-27b.hard` (p_value)
\tjset{jb_gate_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.deepseek-flash.all` (ours_only)
\tjset{jb_gate_vs_deepseekflash_all_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.deepseek-flash.all` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_all_p}{$p = 0.754$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.deepseek-flash.all` (p_value)
\tjset{jb_gate_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.deepseek-flash.hard` (ours_only)
\tjset{jb_gate_vs_deepseekflash_hard_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.deepseek-flash.hard` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_hard_p}{$p = 0.508$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.deepseek-flash.hard` (p_value)
\tjset{jb_gate_vs_gpt56luna_all_ours}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (ours_only)
\tjset{jb_gate_vs_gpt56luna_all_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_all_p}{$p = 1.000$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (p_value)
\tjset{jb_gate_vs_gpt56luna_hard_ours}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_gate_vs_gpt56luna_hard_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_hard_p}{$p = 0.508$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (p_value)
\tjset{jb_anytime_correct}{224} % `jevbench-qwen3.5-27b-report-v2.json` `policies.anytime` (correct)
\tjset{jb_anytime_acc}{97.0\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.anytime` (accuracy)
\tjset{jb_anytime_hard_correct}{104} % `jevbench-qwen3.5-27b-report-v2.json` `policies.anytime` (by_tier.hard.correct)
\tjset{jb_anytime_hard_acc}{93.7\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.anytime` (by_tier.hard.accuracy)
\tjset{jb_anytime_ece}{0.043} % `jevbench-qwen3.5-27b-report-v2.json` `policies.anytime` (ece)
\tjset{jb_anytime_think}{586} % `jevbench-qwen3.5-27b-report-v2.json` `policies.anytime` (mean_think_tokens)
\tjset{jb_anytime_escalation}{30.3\%} % `jevbench-qwen3.5-27b-report-v2.json` `policies.anytime` (escalation_rate)
\tjset{jb_anytime_vs_jev1130_all_ours}{26} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.jev-1.13.0.all` (ours_only)
\tjset{jb_anytime_vs_jev1130_all_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.jev-1.13.0.all` (theirs_only)
\tjset{jb_anytime_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.jev-1.13.0.all` (p_value)
\tjset{jb_anytime_vs_jev1130_hard_ours}{25} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (ours_only)
\tjset{jb_anytime_vs_jev1130_hard_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (theirs_only)
\tjset{jb_anytime_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (p_value)
\tjset{jb_anytime_vs_openjevthinking_all_ours}{20} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.openjev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_all_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.openjev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.openjev-thinking.all` (p_value)
\tjset{jb_anytime_vs_openjevthinking_hard_ours}{20} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.openjev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_hard_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.openjev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.openjev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_djevthinking_all_ours}{27} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.djev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_djevthinking_all_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.djev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.djev-thinking.all` (p_value)
\tjset{jb_anytime_vs_djevthinking_hard_ours}{24} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.djev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_djevthinking_hard_theirs}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.djev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.djev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_all_ours}{38} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_all_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_hard_ours}{37} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_theirs}{1} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_anytime_vs_reflex27b_all_ours}{25} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.reflex-27b.all` (ours_only)
\tjset{jb_anytime_vs_reflex27b_all_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.reflex-27b.all` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.reflex-27b.all` (p_value)
\tjset{jb_anytime_vs_reflex27b_hard_ours}{22} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.reflex-27b.hard` (ours_only)
\tjset{jb_anytime_vs_reflex27b_hard_theirs}{2} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.reflex-27b.hard` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.reflex-27b.hard` (p_value)
\tjset{jb_anytime_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.deepseek-flash.all` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_all_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.deepseek-flash.all` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_all_p}{$p = 0.754$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.deepseek-flash.all` (p_value)
\tjset{jb_anytime_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.deepseek-flash.hard` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_hard_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.deepseek-flash.hard` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_hard_p}{$p = 0.508$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.deepseek-flash.hard` (p_value)
\tjset{jb_anytime_vs_gpt56luna_all_ours}{5} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_all_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_all_p}{$p = 1.000$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (p_value)
\tjset{jb_anytime_vs_gpt56luna_hard_ours}{3} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_hard_theirs}{6} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_hard_p}{$p = 0.508$} % `jevbench-qwen3.5-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (p_value)
\tjset{jb_sys_jev1130_correct}{200} % `jevbench-qwen3.5-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (correct)
\tjset{jb_sys_jev1130_acc}{86.6\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_jev1130_hard_correct}{81} % `jevbench-qwen3.5-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_jev1130_hard_acc}{73.0\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_openjevthinking_correct}{205} % `jevbench-qwen3.5-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_openjevthinking_acc}{88.7\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_openjevthinking_hard_correct}{85} % `jevbench-qwen3.5-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_openjevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_djevthinking_correct}{202} % `jevbench-qwen3.5-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_djevthinking_acc}{87.4\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_djevthinking_hard_correct}{85} % `jevbench-qwen3.5-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_djevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_semifqwen354b_correct}{187} % `jevbench-qwen3.5-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (correct)
\tjset{jb_sys_semifqwen354b_acc}{81.0\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_semifqwen354b_hard_correct}{68} % `jevbench-qwen3.5-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_semifqwen354b_hard_acc}{61.3\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_reflex27b_correct}{201} % `jevbench-qwen3.5-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (correct)
\tjset{jb_sys_reflex27b_acc}{87.0\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_reflex27b_hard_correct}{84} % `jevbench-qwen3.5-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_reflex27b_hard_acc}{75.7\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_deepseekflash_correct}{226} % `jevbench-qwen3.5-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (correct)
\tjset{jb_sys_deepseekflash_acc}{97.8\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_deepseekflash_hard_correct}{107} % `jevbench-qwen3.5-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_deepseekflash_hard_acc}{96.4\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_gpt56luna_correct}{225} % `jevbench-qwen3.5-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (correct)
\tjset{jb_sys_gpt56luna_acc}{97.4\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_gpt56luna_hard_correct}{107} % `jevbench-qwen3.5-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_gpt56luna_hard_acc}{96.4\%} % `jevbench-qwen3.5-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_rows}{231} % `jevbench-qwen3.5-27b-report-v2.json` `policies.*.n`
\tjset{jb_hard_rows}{111} % `jevbench-qwen3.5-27b-report-v2.json` `policies.*.by_tier.hard.n`


==> figures/qwen3.5-27b/per_source.tex <==
A & Escalation (CLINC) & en & -- & 290 & 60.0\% & 72.4\% & 71.0\% & 43.1\% \\
A & Every judgments & en & -- & 84 & 95.2\% & 95.2\% & 95.2\% & 7.1\% \\
A & Intent routing (BANKING77) & en & -- & 486 & 85.0\% & 86.4\% & 86.4\% & 18.9\% \\
A & Intent routing (CLINC) & en & -- & 358 & 95.5\% & 97.5\% & 97.2\% & 9.8\% \\
A & NLI (WANLI) & en & -- & 159 & 75.5\% & 81.1\% & 79.2\% & 32.7\% \\
A & SemIf authored & en & -- & 84 & 92.9\% & 94.0\% & 95.2\% & 10.7\% \\
A & Typed decisions & en & -- & 1165 & 71.2\% & 73.3\% & 73.7\% & 61.5\% \\
\midrule
B & BIG-Bench Hard & en & -- & 620 & 70.6\% & 94.8\% & 94.4\% & 53.9\% \\
B & GPQA Diamond & en & -- & 117 & 60.7\% & 85.5\% & 85.5\% & 78.6\% \\
B & MMLU-Pro & en & -- & 715 & 56.9\% & 82.9\% & 82.8\% & 71.9\% \\
B & MuSR & en & -- & 383 & 62.1\% & 68.9\% & 68.7\% & 51.2\% \\
B & SuperGPQA & en & -- & 652 & 47.7\% & 62.1\% & 62.0\% & 83.4\% \\
\midrule
C & Chess (Lichess) & en & 1 & 121 & 64.5\% & 71.1\% & 71.1\% & 92.6\% \\
C & Chess (Lichess) & en & 2 & 125 & 34.4\% & 42.4\% & 42.4\% & 98.4\% \\
C & Chess (Lichess) & en & 3 & 126 & 34.9\% & 37.3\% & 37.3\% & 100.0\% \\
C & Chess (Lichess) & en & 4 & 122 & 32.8\% & 37.7\% & 37.7\% & 100.0\% \\
C & Chess (Lichess) & zh & 1 & 58 & 50.0\% & 58.6\% & 58.6\% & 91.4\% \\
C & Chess (Lichess) & zh & 2 & 59 & 40.7\% & 40.7\% & 40.7\% & 100.0\% \\
C & Chess (Lichess) & zh & 3 & 60 & 33.3\% & 46.7\% & 46.7\% & 100.0\% \\
C & Chess (Lichess) & zh & 4 & 62 & 29.0\% & 29.0\% & 29.0\% & 100.0\% \\
C & Generated families & en & 1 & 356 & 69.9\% & 100.0\% & 99.4\% & 49.4\% \\
C & Generated families & en & 2 & 362 & 66.6\% & 100.0\% & 93.1\% & 60.8\% \\
C & Generated families & en & 3 & 358 & 39.7\% & 100.0\% & 95.8\% & 84.1\% \\
C & Generated families & en & 4 & 369 & 40.7\% & 98.1\% & 95.7\% & 91.9\% \\
C & Generated families & zh & 1 & 232 & 66.8\% & 100.0\% & 99.1\% & 51.3\% \\
C & Generated families & zh & 2 & 245 & 64.5\% & 100.0\% & 95.5\% & 67.3\% \\
C & Generated families & zh & 3 & 247 & 44.1\% & 100.0\% & 96.0\% & 87.9\% \\
C & Generated families & zh & 4 & 223 & 43.5\% & 98.7\% & 96.4\% & 92.8\% \\
C & hard200 fixture & en & -- & 121 & 82.6\% & 100.0\% & 95.9\% & 34.7\% \\


==> figures/qwen3.5-4b/data.tex <==
A & Escalation (CLINC) & 210 & 290 & en & CC-BY-3.0 \\
A & Every judgments & 70 & 84 & en & unstated \\
A & Intent routing (BANKING77) & 313 & 486 & en & CC-BY-4.0 \\
A & Intent routing (CLINC) & 242 & 358 & en & CC-BY-3.0 \\
A & NLI (WANLI) & 97 & 159 & en & CC-BY-4.0 \\
A & SemIf authored & 60 & 84 & en & MIT \\
A & Typed decisions & 835 & 1165 & en & Apache-2.0 \\
\midrule
B & BIG-Bench Hard & 400 & 620 & en & MIT \\
B & GPQA Diamond & 81 & 117 & en & CC-BY-4.0 \\
B & MMLU-Pro & 475 & 715 & en & MIT \\
B & MuSR & 217 & 383 & en & CC-BY-4.0 \\
B & SuperGPQA & 428 & 652 & en & ODC-BY-1.0 \\
\midrule
C & Chess (Lichess) & 467 & 733 & en, zh & CC0-1.0 \\
C & Generated families & 1608 & 2392 & en, zh & MIT \\
C & hard200 fixture & 79 & 121 & en & MIT \\
\midrule
All & & 5582 & 8359 & & \\


==> figures/qwen3.5-4b/numbers.tex <==
\tjset{rows_test}{8359} % `rows.test`
\tjset{always_s1_accuracy}{50.9\%} % `baselines_test.always_s1_accuracy`
\tjset{always_s2_accuracy}{77.4\%} % `baselines_test.always_s2_accuracy`
\tjset{always_s2_mean_think_tokens}{2126} % `baselines_test.s2_mean_think_tokens`
\tjset{s1_wrong_s2_right}{2560} % `baselines_test.s1_wrong_s2_right`
\tjset{s1_right_s2_wrong}{340} % `baselines_test.s1_right_s2_wrong`
\tjset{s1_ece}{0.029} % `s1_readouts_test.*.ece`
\tjset{gate_test_accuracy}{76.5\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_mean_think_tokens}{1822} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_thinking_share}{86\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{anytime_test_accuracy}{76.5\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_mean_think_tokens}{1763} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_thinking_share}{83\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{s1_ltt_coverage_at_5pct}{6.5\%} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_5pct}{1.1\%} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_risk)
\tjset{block_all_rows}{8359} % `per_family_test` (rows, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s1}{50.9\%} % `per_family_test` (s1_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s2}{77.4\%} % `per_family_test` (s2_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_system}{76.4\%} % `per_family_test` (system_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_escalation}{71.6\%} % `per_family_test` (escalation_rate, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_jev_rows}{2626} % `per_family_test` (rows, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s1}{72.2\%} % `per_family_test` (s1_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s2}{79.4\%} % `per_family_test` (s2_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_system}{77.8\%} % `per_family_test` (system_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_escalation}{39.2\%} % `per_family_test` (escalation_rate, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_public_rows}{2487} % `per_family_test` (rows, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s1}{42.2\%} % `per_family_test` (s1_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s2}{68.4\%} % `per_family_test` (s2_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_system}{67.8\%} % `per_family_test` (system_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_escalation}{78.3\%} % `per_family_test` (escalation_rate, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_weak_rows}{3246} % `per_family_test` (rows, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s1}{40.3\%} % `per_family_test` (s1_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s2}{82.8\%} % `per_family_test` (s2_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_system}{81.9\%} % `per_family_test` (system_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_escalation}{92.6\%} % `per_family_test` (escalation_rate, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{oracle_accuracy}{81.5\%} % `baselines_test.oracle_best_accuracy`
\tjset{s2_closed_naturally}{73.4\%} % `baselines_test.s2_closed_naturally_rate`
\tjset{disagree_total}{2900} % `baselines_test.s1_wrong_s2_right` + `s1_right_s2_wrong`
\tjset{h2_accuracy}{76.4\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{h2_gap}{1.0} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, always-S2 accuracy minus test_accuracy, in points)
\tjset{h2_escalation}{71.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{s1_raw_accuracy}{50.9\%} % `s1_readouts_test.raw.accuracy`
\tjset{s1_raw_ece}{0.024} % `s1_readouts_test.raw.ece`
\tjset{s1_rotation_accuracy}{54.6\%} % `s1_readouts_test.rotation.accuracy`
\tjset{s1_rotation_ece}{0.029} % `s1_readouts_test.rotation.ece`
\tjset{s1_ece_uncalibrated}{0.068} % `s1_readouts_test.rotation.ece_t1`
\tjset{s1_prior_accuracy}{55.1\%} % `s1_readouts_test.rotation_batch_prior.accuracy`
\tjset{s1_prior_ece}{0.044} % `s1_readouts_test.rotation_batch_prior.ece`
\tjset{s1_order_flip_rate}{55.9\%} % `order_flip_rate_test.all`
\tjset{temp_s1}{1.44} % `s1_readouts_test.rotation.temperature`
\tjset{s1_ltt_coverage_at_1pct}{0.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_1pct}{--} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_risk)
\tjset{s1_ltt_interval_at_1pct}{} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_2pct}{0.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_2pct}{--} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_risk)
\tjset{s1_ltt_interval_at_2pct}{} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_interval_at_5pct}{[0.4, 2.4]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.05, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_10pct}{16.6\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_10pct}{8.3\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_risk)
\tjset{s1_ltt_interval_at_10pct}{[6.9, 9.9]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_targets_certified}{2} % `s1_readouts_test.rotation.coverage_at_risk` (targets with ltt_test_coverage > 0)
\tjset{anytime_acc_t0}{51.5\%} % `anytime_test.per_checkpoint` (t = 0, accuracy)
\tjset{anytime_ece_t0}{0.016} % `anytime_test.per_checkpoint` (t = 0, ece)
\tjset{anytime_tokens_t0}{0} % `anytime_test.per_checkpoint` (t = 0, mean_think_tokens)
\tjset{anytime_acc_t128}{51.8\%} % `anytime_test.per_checkpoint` (t = 128, accuracy)
\tjset{anytime_ece_t128}{0.021} % `anytime_test.per_checkpoint` (t = 128, ece)
\tjset{anytime_tokens_t128}{128} % `anytime_test.per_checkpoint` (t = 128, mean_think_tokens)
\tjset{anytime_acc_t256}{52.8\%} % `anytime_test.per_checkpoint` (t = 256, accuracy)
\tjset{anytime_ece_t256}{0.020} % `anytime_test.per_checkpoint` (t = 256, ece)
\tjset{anytime_tokens_t256}{256} % `anytime_test.per_checkpoint` (t = 256, mean_think_tokens)
\tjset{anytime_acc_t512}{58.6\%} % `anytime_test.per_checkpoint` (t = 512, accuracy)
\tjset{anytime_ece_t512}{0.016} % `anytime_test.per_checkpoint` (t = 512, ece)
\tjset{anytime_tokens_t512}{505} % `anytime_test.per_checkpoint` (t = 512, mean_think_tokens)
\tjset{anytime_acc_t1024}{68.4\%} % `anytime_test.per_checkpoint` (t = 1024, accuracy)
\tjset{anytime_ece_t1024}{0.040} % `anytime_test.per_checkpoint` (t = 1024, ece)
\tjset{anytime_tokens_t1024}{890} % `anytime_test.per_checkpoint` (t = 1024, mean_think_tokens)
\tjset{anytime_acc_t2048}{74.9\%} % `anytime_test.per_checkpoint` (t = 2048, accuracy)
\tjset{anytime_ece_t2048}{0.031} % `anytime_test.per_checkpoint` (t = 2048, ece)
\tjset{anytime_tokens_t2048}{1415} % `anytime_test.per_checkpoint` (t = 2048, mean_think_tokens)
\tjset{anytime_acc_full}{77.4\%} % `anytime_test.full_thought.accuracy`
\tjset{anytime_ece_full}{0.031} % `anytime_test.full_thought.ece`
\tjset{temp_t0}{1.61} % `anytime_test.per_checkpoint` (t = 0, temperature)
\tjset{temp_t128}{1.66} % `anytime_test.per_checkpoint` (t = 128, temperature)
\tjset{temp_t256}{1.70} % `anytime_test.per_checkpoint` (t = 256, temperature)
\tjset{temp_t512}{2.05} % `anytime_test.per_checkpoint` (t = 512, temperature)
\tjset{temp_t1024}{2.89} % `anytime_test.per_checkpoint` (t = 1024, temperature)
\tjset{temp_t2048}{3.39} % `anytime_test.per_checkpoint` (t = 2048, temperature)
\tjset{temp_full}{3.78} % `anytime_test.full_thought.temperature`
\tjset{gate_eps0_accuracy}{77.4\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_accuracy)
\tjset{gate_eps0_escalation}{89.7\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, 1 - test_coverage)
\tjset{gate_eps0_share}{97\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps0_accuracy}{77.4\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_accuracy)
\tjset{anytime_eps0_share}{97\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps1_accuracy}{76.4\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{gate_eps1_escalation}{71.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{gate_eps1_share}{85\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps1_accuracy}{76.5\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_accuracy)
\tjset{anytime_eps1_share}{83\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps2_accuracy}{75.5\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_accuracy)
\tjset{gate_eps2_escalation}{63.9\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, 1 - test_coverage)
\tjset{gate_eps2_share}{77\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps2_accuracy}{75.9\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_accuracy)
\tjset{anytime_eps2_share}{76\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{stop_s1}{23.8\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered by S1
\tjset{stop_checkpoint}{19.5\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered at a checkpoint before the full thought
\tjset{stop_full}{56.7\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered after the full thought
\tjset{stop_checkpoint_of_escalated}{25.6\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of escalated rows that stop at a checkpoint
\tjset{lang_en_rows}{1445} % `per_family_test` (rows, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s1}{40.9\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s2}{96.1\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_system}{94.9\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_escalation}{92.1\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'en')
\tjset{lang_zh_rows}{947} % `per_family_test` (rows, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s1}{41.0\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s2}{96.0\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_system}{94.8\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_escalation}{91.4\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'zh')
\tjset{combined_eps0_accuracy}{77.4\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_accuracy)
\tjset{combined_eps0_escalation}{88.8\%} % `dev_selected_operating_points` (combined, tolerance 0.0, 1 - test_coverage)
\tjset{combined_eps0_share}{96\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps1_accuracy}{76.4\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_accuracy)
\tjset{combined_eps1_escalation}{71.9\%} % `dev_selected_operating_points` (combined, tolerance 0.01, 1 - test_coverage)
\tjset{combined_eps1_share}{85\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps2_accuracy}{75.3\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_accuracy)
\tjset{combined_eps2_escalation}{61.5\%} % `dev_selected_operating_points` (combined, tolerance 0.02, 1 - test_coverage)
\tjset{combined_eps2_share}{75\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_weight_confidence_rot}{1.106} % `combined_fit.standardized_weights.confidence_rot`
\tjset{combined_weight_router_zero_shot}{0.164} % `combined_fit.standardized_weights.router_zero_shot`
\tjset{auroc_confidence}{0.765} % `auroc_s1_correct_test.confidence`
\tjset{auroc_confidence_rot}{0.757} % `auroc_s1_correct_test.confidence_rot`
\tjset{auroc_probe}{0.781} % `auroc_s1_correct_test.probe`
\tjset{auroc_router_probe}{0.762} % `auroc_s1_correct_test.router_probe`
\tjset{auroc_router_zero_shot}{0.688} % `auroc_s1_correct_test.router_zero_shot`
\tjset{auroc_router_supervised}{0.683} % `auroc_s1_correct_test.router_supervised`
\tjset{auroc_combined}{0.756} % `auroc_s1_correct_test.combined`
\tjset{area_confidence}{0.347} % `normalized_area_test.area.confidence`
\tjset{area_confidence_rot}{0.360} % `normalized_area_test.area.confidence_rot`
\tjset{area_probe}{0.344} % `normalized_area_test.area.probe`
\tjset{area_router_probe}{0.317} % `normalized_area_test.area.router_probe`
\tjset{area_router_zero_shot}{0.349} % `normalized_area_test.area.router_zero_shot`
\tjset{area_router_supervised}{0.199} % `normalized_area_test.area.router_supervised`
\tjset{area_combined}{0.378} % `normalized_area_test.area.combined`
\tjset{area_diff_confidence}{+0.013} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_confidence}{[$-$0.009, +0.037]} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, ci95)
\tjset{area_diff_probe}{+0.017} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_probe}{[$-$0.010, +0.040]} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_probe}{+0.043} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_probe}{[+0.018, +0.068]} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_zero_shot}{+0.011} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_zero_shot}{[$-$0.017, +0.037]} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_supervised}{+0.161} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_supervised}{[+0.133, +0.190]} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, ci95)
\tjset{area_diff_combined}{$-$0.018} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_combined}{[$-$0.023, $-$0.013]} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, ci95)
\tjset{disagree_jev_fix}{315} % `disagreement_test.by_source` (summed over block 'jev', s1_wrong_s2_right)
\tjset{disagree_jev_break}{127} % `disagreement_test.by_source` (summed over block 'jev', s1_right_s2_wrong)
\tjset{disagree_public_fix}{759} % `disagreement_test.by_source` (summed over block 'public', s1_wrong_s2_right)
\tjset{disagree_public_break}{106} % `disagreement_test.by_source` (summed over block 'public', s1_right_s2_wrong)
\tjset{disagree_weak_fix}{1486} % `disagreement_test.by_source` (summed over block 'weak', s1_wrong_s2_right)
\tjset{disagree_weak_break}{107} % `disagreement_test.by_source` (summed over block 'weak', s1_right_s2_wrong)
\tjset{grp_arithmetic_rows}{288} % `per_family_test` (rows, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s1}{30.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_escalation}{100.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Arithmetic')
\tjset{grp_datecomparison_rows}{293} % `per_family_test` (rows, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s1}{33.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s2}{87.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_system}{87.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_escalation}{100.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date comparison')
\tjset{grp_chess_rows}{733} % `per_family_test` (rows, row-weighted over group 'Chess')
\tjset{grp_chess_s1}{34.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_s2}{37.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_system}{37.1\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_escalation}{99.5\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chess')
\tjset{grp_logicgrid_rows}{272} % `per_family_test` (rows, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s1}{34.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s2}{95.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_system}{95.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_escalation}{99.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'Logic grid')
\tjset{grp_scheduling_rows}{301} % `per_family_test` (rows, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s1}{42.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s2}{98.3\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_system}{97.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_escalation}{92.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Scheduling')
\tjset{grp_graphpaths_rows}{313} % `per_family_test` (rows, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s1}{43.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s2}{94.9\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_system}{89.1\%} % `per_family_test` (system_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_escalation}{80.2\%} % `per_family_test` (escalation_rate, row-weighted over group 'Graph paths')
\tjset{grp_chainedrules_rows}{298} % `per_family_test` (rows, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s1}{43.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s2}{99.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_system}{99.3\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_escalation}{97.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chained rules')
\tjset{grp_counting_rows}{345} % `per_family_test` (rows, row-weighted over group 'Counting')
\tjset{grp_counting_s1}{44.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_system}{99.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_escalation}{93.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'Counting')
\tjset{grp_stackednegation_rows}{315} % `per_family_test` (rows, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s1}{54.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s2}{92.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_system}{91.1\%} % `per_family_test` (system_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_escalation}{74.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Stacked negation')
\tjset{grp_datedeadlines_rows}{27} % `per_family_test` (rows, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s1}{55.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_escalation}{96.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date deadlines')
\tjset{grp_doublenegationhard200_rows}{30} % `per_family_test` (rows, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s1}{70.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s2}{90.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_system}{80.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_escalation}{16.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Double negation (hard200)')
\tjset{grp_multihopruleshard200_rows}{31} % `per_family_test` (rows, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s1}{80.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_escalation}{48.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_typeddecisions_rows}{1165} % `per_family_test` (rows, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s1}{63.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s2}{71.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_system}{70.3\%} % `per_family_test` (system_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_escalation}{59.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'Typed decisions')
\tjset{grp_nliwanli_rows}{159} % `per_family_test` (rows, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s1}{64.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s2}{73.6\%} % `per_family_test` (s2_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_system}{69.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_escalation}{35.2\%} % `per_family_test` (escalation_rate, row-weighted over group 'NLI (WANLI)')
\tjset{grp_escalationclinc_rows}{290} % `per_family_test` (rows, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s1}{69.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s2}{84.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_system}{77.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_escalation}{34.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_intentroutingbanking77_rows}{486} % `per_family_test` (rows, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s1}{79.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s2}{81.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_system}{80.5\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_escalation}{21.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_semifauthored_rows}{84} % `per_family_test` (rows, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s1}{82.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s2}{95.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_system}{94.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_escalation}{23.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'SemIf authored')
\tjset{grp_intentroutingclinc_rows}{358} % `per_family_test` (rows, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s1}{89.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s2}{95.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_system}{95.3\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_escalation}{15.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_everyjudgments_rows}{84} % `per_family_test` (rows, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s1}{96.4\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s2}{95.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_system}{94.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_escalation}{4.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'Every judgments')
\tjset{grp_supergpqa_rows}{652} % `per_family_test` (rows, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s1}{29.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s2}{45.4\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_system}{44.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_escalation}{88.5\%} % `per_family_test` (escalation_rate, row-weighted over group 'SuperGPQA')
\tjset{grp_gpqadiamond_rows}{117} % `per_family_test` (rows, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s1}{30.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s2}{71.8\%} % `per_family_test` (s2_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_system}{71.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_escalation}{95.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'GPQA Diamond')
\tjset{grp_mmlupro_rows}{715} % `per_family_test` (rows, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s1}{37.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s2}{73.6\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_system}{73.1\%} % `per_family_test` (system_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_escalation}{83.2\%} % `per_family_test` (escalation_rate, row-weighted over group 'MMLU-Pro')
\tjset{grp_musr_rows}{383} % `per_family_test` (rows, row-weighted over group 'MuSR')
\tjset{grp_musr_s1}{53.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_s2}{62.4\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_system}{61.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_escalation}{55.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'MuSR')
\tjset{grp_bigbenchhard_rows}{620} % `per_family_test` (rows, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s1}{55.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s2}{89.8\%} % `per_family_test` (s2_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_system}{89.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_escalation}{72.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'BIG-Bench Hard')
\tjset{difficulty_families}{9} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty computed per family)
\tjset{difficulty_rising}{7} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty > 0)
\tjset{weak_d1_rows}{767} % `per_family_test` (rows, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_escalation}{81.5\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s1}{54.0\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s2}{90.0\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d2_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_escalation}{93.8\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s1}{40.8\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s2}{82.7\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d3_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_escalation}{99.2\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s1}{31.2\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s2}{80.0\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d4_rows}{776} % `per_family_test` (rows, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_escalation}{99.7\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s1}{31.4\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s2}{76.4\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 4)
\tjset{lat_rows}{600} % `qwen3.5-4b-latency.jsonl` (rows)
\tjset{lat_prefix_tokens}{261} % `qwen3.5-4b-latency.jsonl` (median prefix_tokens)
\tjset{lat_prefill_ms}{101} % `qwen3.5-4b-latency.jsonl` (median prefill_seconds, ms)
\tjset{lat_copy_ms}{4} % `qwen3.5-4b-latency.jsonl` (median copy_seconds, ms)
\tjset{lat_s1_ms}{50} % `qwen3.5-4b-latency.jsonl` (median s1_seconds, ms)
\tjset{lat_rotation_ms}{164} % `qwen3.5-4b-latency.jsonl` (median rotation_seconds, ms)
\tjset{lat_s1_marginal_ms}{53} % `qwen3.5-4b-latency.jsonl` (median copy_seconds + s1_seconds, ms)
\tjset{lat_s2_seconds}{30.3} % `qwen3.5-4b-latency.jsonl` (median s2_seconds)
\tjset{lat_s2_think_tokens}{1038} % `qwen3.5-4b-latency.jsonl` (median s2_think_tokens)
\tjset{jb_s1_correct}{185} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s1` (correct)
\tjset{jb_s1_acc}{80.1\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s1` (accuracy)
\tjset{jb_s1_hard_correct}{69} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s1` (by_tier.hard.correct)
\tjset{jb_s1_hard_acc}{62.2\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s1` (by_tier.hard.accuracy)
\tjset{jb_s1_ece}{0.060} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s1` (ece)
\tjset{jb_s1_think}{0} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s1` (mean_think_tokens)
\tjset{jb_s1_escalation}{0.0\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s1` (escalation_rate)
\tjset{jb_s1_vs_jev1130_all_ours}{9} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.jev-1.13.0.all` (ours_only)
\tjset{jb_s1_vs_jev1130_all_theirs}{24} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.jev-1.13.0.all` (theirs_only)
\tjset{jb_s1_vs_jev1130_all_p}{$p = 0.014$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.jev-1.13.0.all` (p_value)
\tjset{jb_s1_vs_jev1130_hard_ours}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.jev-1.13.0.hard` (ours_only)
\tjset{jb_s1_vs_jev1130_hard_theirs}{20} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s1_vs_jev1130_hard_p}{$p = 0.036$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.jev-1.13.0.hard` (p_value)
\tjset{jb_s1_vs_openjevthinking_all_ours}{9} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.openjev-thinking.all` (ours_only)
\tjset{jb_s1_vs_openjevthinking_all_theirs}{29} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.openjev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_all_p}{$p = 0.002$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.openjev-thinking.all` (p_value)
\tjset{jb_s1_vs_openjevthinking_hard_ours}{9} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.openjev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_openjevthinking_hard_theirs}{25} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.openjev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_hard_p}{$p = 0.009$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.openjev-thinking.hard` (p_value)
\tjset{jb_s1_vs_djevthinking_all_ours}{18} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.djev-thinking.all` (ours_only)
\tjset{jb_s1_vs_djevthinking_all_theirs}{35} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.djev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_djevthinking_all_p}{$p = 0.027$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.djev-thinking.all` (p_value)
\tjset{jb_s1_vs_djevthinking_hard_ours}{15} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.djev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_djevthinking_hard_theirs}{31} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.djev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_djevthinking_hard_p}{$p = 0.026$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.djev-thinking.hard` (p_value)
\tjset{jb_s1_vs_semifqwen354b_all_ours}{9} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_all_theirs}{11} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_all_p}{$p = 0.824$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s1_vs_semifqwen354b_hard_ours}{9} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_hard_theirs}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_hard_p}{$p = 1.000$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s1_vs_reflex27b_all_ours}{9} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.reflex-27b.all` (ours_only)
\tjset{jb_s1_vs_reflex27b_all_theirs}{25} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.reflex-27b.all` (theirs_only)
\tjset{jb_s1_vs_reflex27b_all_p}{$p = 0.009$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.reflex-27b.all` (p_value)
\tjset{jb_s1_vs_reflex27b_hard_ours}{7} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.reflex-27b.hard` (ours_only)
\tjset{jb_s1_vs_reflex27b_hard_theirs}{22} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.reflex-27b.hard` (theirs_only)
\tjset{jb_s1_vs_reflex27b_hard_p}{$p = 0.008$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.reflex-27b.hard` (p_value)
\tjset{jb_s1_vs_deepseekflash_all_ours}{3} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.deepseek-flash.all` (ours_only)
\tjset{jb_s1_vs_deepseekflash_all_theirs}{44} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.deepseek-flash.all` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_all_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.deepseek-flash.all` (p_value)
\tjset{jb_s1_vs_deepseekflash_hard_ours}{2} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.deepseek-flash.hard` (ours_only)
\tjset{jb_s1_vs_deepseekflash_hard_theirs}{40} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.deepseek-flash.hard` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.deepseek-flash.hard` (p_value)
\tjset{jb_s1_vs_gpt56luna_all_ours}{3} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s1_vs_gpt56luna_all_theirs}{43} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_all_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (p_value)
\tjset{jb_s1_vs_gpt56luna_hard_ours}{1} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s1_vs_gpt56luna_hard_theirs}{39} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (p_value)
\tjset{jb_s2_correct}{215} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s2` (correct)
\tjset{jb_s2_acc}{93.1\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s2` (accuracy)
\tjset{jb_s2_hard_correct}{95} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s2` (by_tier.hard.correct)
\tjset{jb_s2_hard_acc}{85.6\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s2` (by_tier.hard.accuracy)
\tjset{jb_s2_ece}{0.064} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s2` (ece)
\tjset{jb_s2_think}{1530} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s2` (mean_think_tokens)
\tjset{jb_s2_escalation}{100.0\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.s2` (escalation_rate)
\tjset{jb_s2_vs_jev1130_all_ours}{21} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.jev-1.13.0.all` (ours_only)
\tjset{jb_s2_vs_jev1130_all_theirs}{6} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.jev-1.13.0.all` (theirs_only)
\tjset{jb_s2_vs_jev1130_all_p}{$p = 0.006$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.jev-1.13.0.all` (p_value)
\tjset{jb_s2_vs_jev1130_hard_ours}{20} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.jev-1.13.0.hard` (ours_only)
\tjset{jb_s2_vs_jev1130_hard_theirs}{6} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s2_vs_jev1130_hard_p}{$p = 0.009$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.jev-1.13.0.hard` (p_value)
\tjset{jb_s2_vs_openjevthinking_all_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.openjev-thinking.all` (ours_only)
\tjset{jb_s2_vs_openjevthinking_all_theirs}{6} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.openjev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_all_p}{$p = 0.052$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.openjev-thinking.all` (p_value)
\tjset{jb_s2_vs_openjevthinking_hard_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.openjev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_openjevthinking_hard_theirs}{6} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.openjev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_hard_p}{$p = 0.052$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.openjev-thinking.hard` (p_value)
\tjset{jb_s2_vs_djevthinking_all_ours}{25} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.djev-thinking.all` (ours_only)
\tjset{jb_s2_vs_djevthinking_all_theirs}{12} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.djev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_djevthinking_all_p}{$p = 0.047$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.djev-thinking.all` (p_value)
\tjset{jb_s2_vs_djevthinking_hard_ours}{22} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.djev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_djevthinking_hard_theirs}{12} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.djev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_djevthinking_hard_p}{$p = 0.121$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.djev-thinking.hard` (p_value)
\tjset{jb_s2_vs_semifqwen354b_all_ours}{33} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_all_theirs}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s2_vs_semifqwen354b_hard_ours}{32} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_hard_theirs}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s2_vs_reflex27b_all_ours}{22} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.reflex-27b.all` (ours_only)
\tjset{jb_s2_vs_reflex27b_all_theirs}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.reflex-27b.all` (theirs_only)
\tjset{jb_s2_vs_reflex27b_all_p}{$p = 0.016$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.reflex-27b.all` (p_value)
\tjset{jb_s2_vs_reflex27b_hard_ours}{19} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.reflex-27b.hard` (ours_only)
\tjset{jb_s2_vs_reflex27b_hard_theirs}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.reflex-27b.hard` (theirs_only)
\tjset{jb_s2_vs_reflex27b_hard_p}{$p = 0.052$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.reflex-27b.hard` (p_value)
\tjset{jb_s2_vs_deepseekflash_all_ours}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.deepseek-flash.all` (ours_only)
\tjset{jb_s2_vs_deepseekflash_all_theirs}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.deepseek-flash.all` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_all_p}{$p = 0.027$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.deepseek-flash.all` (p_value)
\tjset{jb_s2_vs_deepseekflash_hard_ours}{4} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.deepseek-flash.hard` (ours_only)
\tjset{jb_s2_vs_deepseekflash_hard_theirs}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.deepseek-flash.hard` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_hard_p}{$p = 0.012$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.deepseek-flash.hard` (p_value)
\tjset{jb_s2_vs_gpt56luna_all_ours}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s2_vs_gpt56luna_all_theirs}{15} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_all_p}{$p = 0.041$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (p_value)
\tjset{jb_s2_vs_gpt56luna_hard_ours}{3} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s2_vs_gpt56luna_hard_theirs}{15} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_hard_p}{$p = 0.008$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (p_value)
\tjset{jb_gate_correct}{211} % `jevbench-qwen3.5-4b-report-v2.json` `policies.gate` (correct)
\tjset{jb_gate_acc}{91.3\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.gate` (accuracy)
\tjset{jb_gate_hard_correct}{93} % `jevbench-qwen3.5-4b-report-v2.json` `policies.gate` (by_tier.hard.correct)
\tjset{jb_gate_hard_acc}{83.8\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.gate` (by_tier.hard.accuracy)
\tjset{jb_gate_ece}{0.082} % `jevbench-qwen3.5-4b-report-v2.json` `policies.gate` (ece)
\tjset{jb_gate_think}{966} % `jevbench-qwen3.5-4b-report-v2.json` `policies.gate` (mean_think_tokens)
\tjset{jb_gate_escalation}{32.9\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.gate` (escalation_rate)
\tjset{jb_gate_vs_jev1130_all_ours}{18} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.jev-1.13.0.all` (ours_only)
\tjset{jb_gate_vs_jev1130_all_theirs}{7} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.jev-1.13.0.all` (theirs_only)
\tjset{jb_gate_vs_jev1130_all_p}{$p = 0.043$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.jev-1.13.0.all` (p_value)
\tjset{jb_gate_vs_jev1130_hard_ours}{17} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.jev-1.13.0.hard` (ours_only)
\tjset{jb_gate_vs_jev1130_hard_theirs}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.jev-1.13.0.hard` (theirs_only)
\tjset{jb_gate_vs_jev1130_hard_p}{$p = 0.017$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.jev-1.13.0.hard` (p_value)
\tjset{jb_gate_vs_openjevthinking_all_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.openjev-thinking.all` (ours_only)
\tjset{jb_gate_vs_openjevthinking_all_theirs}{10} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.openjev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_all_p}{$p = 0.327$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.openjev-thinking.all` (p_value)
\tjset{jb_gate_vs_openjevthinking_hard_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.openjev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_openjevthinking_hard_theirs}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.openjev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_hard_p}{$p = 0.152$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.openjev-thinking.hard` (p_value)
\tjset{jb_gate_vs_djevthinking_all_ours}{23} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.djev-thinking.all` (ours_only)
\tjset{jb_gate_vs_djevthinking_all_theirs}{14} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.djev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_djevthinking_all_p}{$p = 0.188$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.djev-thinking.all` (p_value)
\tjset{jb_gate_vs_djevthinking_hard_ours}{20} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.djev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_djevthinking_hard_theirs}{12} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.djev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_djevthinking_hard_p}{$p = 0.215$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.djev-thinking.hard` (p_value)
\tjset{jb_gate_vs_semifqwen354b_all_ours}{29} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_all_theirs}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_gate_vs_semifqwen354b_hard_ours}{29} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_hard_theirs}{4} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_gate_vs_reflex27b_all_ours}{18} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.reflex-27b.all` (ours_only)
\tjset{jb_gate_vs_reflex27b_all_theirs}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.reflex-27b.all` (theirs_only)
\tjset{jb_gate_vs_reflex27b_all_p}{$p = 0.076$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.reflex-27b.all` (p_value)
\tjset{jb_gate_vs_reflex27b_hard_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.reflex-27b.hard` (ours_only)
\tjset{jb_gate_vs_reflex27b_hard_theirs}{7} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.reflex-27b.hard` (theirs_only)
\tjset{jb_gate_vs_reflex27b_hard_p}{$p = 0.093$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.reflex-27b.hard` (p_value)
\tjset{jb_gate_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.deepseek-flash.all` (ours_only)
\tjset{jb_gate_vs_deepseekflash_all_theirs}{19} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.deepseek-flash.all` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_all_p}{$p = 0.003$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.deepseek-flash.all` (p_value)
\tjset{jb_gate_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.deepseek-flash.hard` (ours_only)
\tjset{jb_gate_vs_deepseekflash_hard_theirs}{17} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.deepseek-flash.hard` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_hard_p}{$p = 0.003$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.deepseek-flash.hard` (p_value)
\tjset{jb_gate_vs_gpt56luna_all_ours}{3} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (ours_only)
\tjset{jb_gate_vs_gpt56luna_all_theirs}{17} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_all_p}{$p = 0.003$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (p_value)
\tjset{jb_gate_vs_gpt56luna_hard_ours}{1} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_gate_vs_gpt56luna_hard_theirs}{15} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (p_value)
\tjset{jb_anytime_correct}{211} % `jevbench-qwen3.5-4b-report-v2.json` `policies.anytime` (correct)
\tjset{jb_anytime_acc}{91.3\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.anytime` (accuracy)
\tjset{jb_anytime_hard_correct}{93} % `jevbench-qwen3.5-4b-report-v2.json` `policies.anytime` (by_tier.hard.correct)
\tjset{jb_anytime_hard_acc}{83.8\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.anytime` (by_tier.hard.accuracy)
\tjset{jb_anytime_ece}{0.069} % `jevbench-qwen3.5-4b-report-v2.json` `policies.anytime` (ece)
\tjset{jb_anytime_think}{986} % `jevbench-qwen3.5-4b-report-v2.json` `policies.anytime` (mean_think_tokens)
\tjset{jb_anytime_escalation}{40.3\%} % `jevbench-qwen3.5-4b-report-v2.json` `policies.anytime` (escalation_rate)
\tjset{jb_anytime_vs_jev1130_all_ours}{18} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.jev-1.13.0.all` (ours_only)
\tjset{jb_anytime_vs_jev1130_all_theirs}{7} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.jev-1.13.0.all` (theirs_only)
\tjset{jb_anytime_vs_jev1130_all_p}{$p = 0.043$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.jev-1.13.0.all` (p_value)
\tjset{jb_anytime_vs_jev1130_hard_ours}{17} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (ours_only)
\tjset{jb_anytime_vs_jev1130_hard_theirs}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (theirs_only)
\tjset{jb_anytime_vs_jev1130_hard_p}{$p = 0.017$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (p_value)
\tjset{jb_anytime_vs_openjevthinking_all_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.openjev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_all_theirs}{10} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.openjev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_all_p}{$p = 0.327$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.openjev-thinking.all` (p_value)
\tjset{jb_anytime_vs_openjevthinking_hard_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.openjev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_hard_theirs}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.openjev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_hard_p}{$p = 0.152$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.openjev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_djevthinking_all_ours}{23} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.djev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_djevthinking_all_theirs}{14} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.djev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_all_p}{$p = 0.188$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.djev-thinking.all` (p_value)
\tjset{jb_anytime_vs_djevthinking_hard_ours}{20} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.djev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_djevthinking_hard_theirs}{12} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.djev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_hard_p}{$p = 0.215$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.djev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_all_ours}{29} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_all_theirs}{5} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_hard_ours}{29} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_theirs}{4} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_anytime_vs_reflex27b_all_ours}{18} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.reflex-27b.all` (ours_only)
\tjset{jb_anytime_vs_reflex27b_all_theirs}{8} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.reflex-27b.all` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_all_p}{$p = 0.076$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.reflex-27b.all` (p_value)
\tjset{jb_anytime_vs_reflex27b_hard_ours}{16} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.reflex-27b.hard` (ours_only)
\tjset{jb_anytime_vs_reflex27b_hard_theirs}{7} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.reflex-27b.hard` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_hard_p}{$p = 0.093$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.reflex-27b.hard` (p_value)
\tjset{jb_anytime_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.deepseek-flash.all` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_all_theirs}{19} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.deepseek-flash.all` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_all_p}{$p = 0.003$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.deepseek-flash.all` (p_value)
\tjset{jb_anytime_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.deepseek-flash.hard` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_hard_theirs}{17} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.deepseek-flash.hard` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_hard_p}{$p = 0.003$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.deepseek-flash.hard` (p_value)
\tjset{jb_anytime_vs_gpt56luna_all_ours}{3} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_all_theirs}{17} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_all_p}{$p = 0.003$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (p_value)
\tjset{jb_anytime_vs_gpt56luna_hard_ours}{1} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_hard_theirs}{15} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-4b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (p_value)
\tjset{jb_sys_jev1130_correct}{200} % `jevbench-qwen3.5-4b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (correct)
\tjset{jb_sys_jev1130_acc}{86.6\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_jev1130_hard_correct}{81} % `jevbench-qwen3.5-4b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_jev1130_hard_acc}{73.0\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_openjevthinking_correct}{205} % `jevbench-qwen3.5-4b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_openjevthinking_acc}{88.7\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_openjevthinking_hard_correct}{85} % `jevbench-qwen3.5-4b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_openjevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_djevthinking_correct}{202} % `jevbench-qwen3.5-4b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_djevthinking_acc}{87.4\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_djevthinking_hard_correct}{85} % `jevbench-qwen3.5-4b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_djevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_semifqwen354b_correct}{187} % `jevbench-qwen3.5-4b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (correct)
\tjset{jb_sys_semifqwen354b_acc}{81.0\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_semifqwen354b_hard_correct}{68} % `jevbench-qwen3.5-4b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_semifqwen354b_hard_acc}{61.3\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_reflex27b_correct}{201} % `jevbench-qwen3.5-4b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (correct)
\tjset{jb_sys_reflex27b_acc}{87.0\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_reflex27b_hard_correct}{84} % `jevbench-qwen3.5-4b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_reflex27b_hard_acc}{75.7\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_deepseekflash_correct}{226} % `jevbench-qwen3.5-4b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (correct)
\tjset{jb_sys_deepseekflash_acc}{97.8\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_deepseekflash_hard_correct}{107} % `jevbench-qwen3.5-4b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_deepseekflash_hard_acc}{96.4\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_gpt56luna_correct}{225} % `jevbench-qwen3.5-4b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (correct)
\tjset{jb_sys_gpt56luna_acc}{97.4\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_gpt56luna_hard_correct}{107} % `jevbench-qwen3.5-4b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_gpt56luna_hard_acc}{96.4\%} % `jevbench-qwen3.5-4b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_rows}{231} % `jevbench-qwen3.5-4b-report-v2.json` `policies.*.n`
\tjset{jb_hard_rows}{111} % `jevbench-qwen3.5-4b-report-v2.json` `policies.*.by_tier.hard.n`


==> figures/qwen3.5-4b/per_source.tex <==
A & Escalation (CLINC) & en & -- & 290 & 69.0\% & 84.1\% & 77.2\% & 34.8\% \\
A & Every judgments & en & -- & 84 & 96.4\% & 95.2\% & 94.0\% & 4.8\% \\
A & Intent routing (BANKING77) & en & -- & 486 & 79.2\% & 81.1\% & 80.5\% & 21.0\% \\
A & Intent routing (CLINC) & en & -- & 358 & 89.9\% & 95.5\% & 95.3\% & 15.9\% \\
A & NLI (WANLI) & en & -- & 159 & 64.2\% & 73.6\% & 69.8\% & 35.2\% \\
A & SemIf authored & en & -- & 84 & 82.1\% & 95.2\% & 94.0\% & 23.8\% \\
A & Typed decisions & en & -- & 1165 & 63.3\% & 71.0\% & 70.3\% & 59.1\% \\
\midrule
B & BIG-Bench Hard & en & -- & 620 & 55.3\% & 89.8\% & 89.0\% & 72.6\% \\
B & GPQA Diamond & en & -- & 117 & 30.8\% & 71.8\% & 71.8\% & 95.7\% \\
B & MMLU-Pro & en & -- & 715 & 37.8\% & 73.6\% & 73.1\% & 83.2\% \\
B & MuSR & en & -- & 383 & 53.8\% & 62.4\% & 61.4\% & 55.6\% \\
B & SuperGPQA & en & -- & 652 & 29.8\% & 45.4\% & 44.8\% & 88.5\% \\
\midrule
C & Chess (Lichess) & en & 1 & 121 & 47.1\% & 55.4\% & 55.4\% & 98.3\% \\
C & Chess (Lichess) & en & 2 & 125 & 34.4\% & 35.2\% & 35.2\% & 99.2\% \\
C & Chess (Lichess) & en & 3 & 126 & 24.6\% & 28.6\% & 28.6\% & 100.0\% \\
C & Chess (Lichess) & en & 4 & 122 & 27.0\% & 29.5\% & 29.5\% & 100.0\% \\
C & Chess (Lichess) & zh & 1 & 58 & 46.6\% & 62.1\% & 62.1\% & 98.3\% \\
C & Chess (Lichess) & zh & 2 & 59 & 28.8\% & 25.4\% & 25.4\% & 100.0\% \\
C & Chess (Lichess) & zh & 3 & 60 & 40.0\% & 35.0\% & 35.0\% & 100.0\% \\
C & Chess (Lichess) & zh & 4 & 62 & 27.4\% & 27.4\% & 27.4\% & 100.0\% \\
C & Generated families & en & 1 & 356 & 55.6\% & 99.7\% & 96.6\% & 77.2\% \\
C & Generated families & en & 2 & 362 & 45.0\% & 97.2\% & 96.1\% & 92.8\% \\
C & Generated families & en & 3 & 358 & 30.4\% & 95.0\% & 94.4\% & 98.6\% \\
C & Generated families & en & 4 & 369 & 32.8\% & 92.7\% & 92.7\% & 99.5\% \\
C & Generated families & zh & 1 & 232 & 56.9\% & 100.0\% & 98.7\% & 75.0\% \\
C & Generated families & zh & 2 & 245 & 40.8\% & 99.2\% & 96.3\% & 91.0\% \\
C & Generated families & zh & 3 & 247 & 33.6\% & 95.5\% & 95.1\% & 99.6\% \\
C & Generated families & zh & 4 & 223 & 32.7\% & 88.8\% & 88.8\% & 100.0\% \\
C & hard200 fixture & en & -- & 121 & 66.9\% & 97.5\% & 95.0\% & 65.3\% \\


==> figures/qwen3.5-9b/data.tex <==
A & Escalation (CLINC) & 210 & 290 & en & CC-BY-3.0 \\
A & Every judgments & 70 & 84 & en & unstated \\
A & Intent routing (BANKING77) & 313 & 486 & en & CC-BY-4.0 \\
A & Intent routing (CLINC) & 242 & 358 & en & CC-BY-3.0 \\
A & NLI (WANLI) & 97 & 159 & en & CC-BY-4.0 \\
A & SemIf authored & 60 & 84 & en & MIT \\
A & Typed decisions & 835 & 1165 & en & Apache-2.0 \\
\midrule
B & BIG-Bench Hard & 400 & 620 & en & MIT \\
B & GPQA Diamond & 81 & 117 & en & CC-BY-4.0 \\
B & MMLU-Pro & 475 & 715 & en & MIT \\
B & MuSR & 217 & 383 & en & CC-BY-4.0 \\
B & SuperGPQA & 428 & 652 & en & ODC-BY-1.0 \\
\midrule
C & Chess (Lichess) & 467 & 733 & en, zh & CC0-1.0 \\
C & Generated families & 1608 & 2392 & en, zh & MIT \\
C & hard200 fixture & 79 & 121 & en & MIT \\
\midrule
All & & 5582 & 8359 & & \\


==> figures/qwen3.5-9b/numbers.tex <==
\tjset{rows_test}{8359} % `rows.test`
\tjset{always_s1_accuracy}{54.1\%} % `baselines_test.always_s1_accuracy`
\tjset{always_s2_accuracy}{80.0\%} % `baselines_test.always_s2_accuracy`
\tjset{always_s2_mean_think_tokens}{2088} % `baselines_test.s2_mean_think_tokens`
\tjset{s1_wrong_s2_right}{2455} % `baselines_test.s1_wrong_s2_right`
\tjset{s1_right_s2_wrong}{292} % `baselines_test.s1_right_s2_wrong`
\tjset{s1_ece}{0.037} % `s1_readouts_test.*.ece`
\tjset{gate_test_accuracy}{79.1\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_mean_think_tokens}{1865} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_thinking_share}{89\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{anytime_test_accuracy}{78.9\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_mean_think_tokens}{1722} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_thinking_share}{82\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{s1_ltt_coverage_at_5pct}{0.0\%} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_5pct}{--} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_risk)
\tjset{block_all_rows}{8359} % `per_family_test` (rows, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s1}{54.1\%} % `per_family_test` (s1_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s2}{80.0\%} % `per_family_test` (s2_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_system}{79.0\%} % `per_family_test` (system_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_escalation}{75.1\%} % `per_family_test` (escalation_rate, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_jev_rows}{2626} % `per_family_test` (rows, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s1}{71.0\%} % `per_family_test` (s1_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s2}{80.4\%} % `per_family_test` (s2_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_system}{78.7\%} % `per_family_test` (system_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_escalation}{47.6\%} % `per_family_test` (escalation_rate, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_public_rows}{2487} % `per_family_test` (rows, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s1}{47.5\%} % `per_family_test` (s1_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s2}{71.8\%} % `per_family_test` (s2_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_system}{71.3\%} % `per_family_test` (system_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_escalation}{82.3\%} % `per_family_test` (escalation_rate, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_weak_rows}{3246} % `per_family_test` (rows, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s1}{45.4\%} % `per_family_test` (s1_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s2}{85.9\%} % `per_family_test` (s2_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_system}{85.2\%} % `per_family_test` (system_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_escalation}{91.7\%} % `per_family_test` (escalation_rate, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{oracle_accuracy}{83.5\%} % `baselines_test.oracle_best_accuracy`
\tjset{s2_closed_naturally}{74.3\%} % `baselines_test.s2_closed_naturally_rate`
\tjset{disagree_total}{2747} % `baselines_test.s1_wrong_s2_right` + `s1_right_s2_wrong`
\tjset{h2_accuracy}{79.0\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{h2_gap}{1.0} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, always-S2 accuracy minus test_accuracy, in points)
\tjset{h2_escalation}{75.1\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{s1_raw_accuracy}{54.1\%} % `s1_readouts_test.raw.accuracy`
\tjset{s1_raw_ece}{0.027} % `s1_readouts_test.raw.ece`
\tjset{s1_rotation_accuracy}{56.5\%} % `s1_readouts_test.rotation.accuracy`
\tjset{s1_rotation_ece}{0.037} % `s1_readouts_test.rotation.ece`
\tjset{s1_ece_uncalibrated}{0.144} % `s1_readouts_test.rotation.ece_t1`
\tjset{s1_prior_accuracy}{56.8\%} % `s1_readouts_test.rotation_batch_prior.accuracy`
\tjset{s1_prior_ece}{0.081} % `s1_readouts_test.rotation_batch_prior.ece`
\tjset{s1_order_flip_rate}{49.1\%} % `order_flip_rate_test.all`
\tjset{temp_s1}{1.82} % `s1_readouts_test.rotation.temperature`
\tjset{s1_ltt_coverage_at_1pct}{0.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_1pct}{--} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_risk)
\tjset{s1_ltt_interval_at_1pct}{} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_2pct}{0.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_2pct}{--} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_risk)
\tjset{s1_ltt_interval_at_2pct}{} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_interval_at_5pct}{} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.05, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_10pct}{17.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_10pct}{6.8\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_risk)
\tjset{s1_ltt_interval_at_10pct}{[5.5, 8.2]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_targets_certified}{1} % `s1_readouts_test.rotation.coverage_at_risk` (targets with ltt_test_coverage > 0)
\tjset{anytime_acc_t0}{53.7\%} % `anytime_test.per_checkpoint` (t = 0, accuracy)
\tjset{anytime_ece_t0}{0.028} % `anytime_test.per_checkpoint` (t = 0, ece)
\tjset{anytime_tokens_t0}{0} % `anytime_test.per_checkpoint` (t = 0, mean_think_tokens)
\tjset{anytime_acc_t128}{54.1\%} % `anytime_test.per_checkpoint` (t = 128, accuracy)
\tjset{anytime_ece_t128}{0.038} % `anytime_test.per_checkpoint` (t = 128, ece)
\tjset{anytime_tokens_t128}{128} % `anytime_test.per_checkpoint` (t = 128, mean_think_tokens)
\tjset{anytime_acc_t256}{55.4\%} % `anytime_test.per_checkpoint` (t = 256, accuracy)
\tjset{anytime_ece_t256}{0.039} % `anytime_test.per_checkpoint` (t = 256, ece)
\tjset{anytime_tokens_t256}{256} % `anytime_test.per_checkpoint` (t = 256, mean_think_tokens)
\tjset{anytime_acc_t512}{62.1\%} % `anytime_test.per_checkpoint` (t = 512, accuracy)
\tjset{anytime_ece_t512}{0.019} % `anytime_test.per_checkpoint` (t = 512, ece)
\tjset{anytime_tokens_t512}{506} % `anytime_test.per_checkpoint` (t = 512, mean_think_tokens)
\tjset{anytime_acc_t1024}{72.2\%} % `anytime_test.per_checkpoint` (t = 1024, accuracy)
\tjset{anytime_ece_t1024}{0.027} % `anytime_test.per_checkpoint` (t = 1024, ece)
\tjset{anytime_tokens_t1024}{892} % `anytime_test.per_checkpoint` (t = 1024, mean_think_tokens)
\tjset{anytime_acc_t2048}{77.7\%} % `anytime_test.per_checkpoint` (t = 2048, accuracy)
\tjset{anytime_ece_t2048}{0.020} % `anytime_test.per_checkpoint` (t = 2048, ece)
\tjset{anytime_tokens_t2048}{1409} % `anytime_test.per_checkpoint` (t = 2048, mean_think_tokens)
\tjset{anytime_acc_full}{80.0\%} % `anytime_test.full_thought.accuracy`
\tjset{anytime_ece_full}{0.023} % `anytime_test.full_thought.ece`
\tjset{temp_t0}{1.63} % `anytime_test.per_checkpoint` (t = 0, temperature)
\tjset{temp_t128}{1.73} % `anytime_test.per_checkpoint` (t = 128, temperature)
\tjset{temp_t256}{1.79} % `anytime_test.per_checkpoint` (t = 256, temperature)
\tjset{temp_t512}{2.00} % `anytime_test.per_checkpoint` (t = 512, temperature)
\tjset{temp_t1024}{2.71} % `anytime_test.per_checkpoint` (t = 1024, temperature)
\tjset{temp_t2048}{3.35} % `anytime_test.per_checkpoint` (t = 2048, temperature)
\tjset{temp_full}{3.80} % `anytime_test.full_thought.temperature`
\tjset{gate_eps0_accuracy}{80.0\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_accuracy)
\tjset{gate_eps0_escalation}{97.1\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, 1 - test_coverage)
\tjset{gate_eps0_share}{99\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps0_accuracy}{80.0\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_accuracy)
\tjset{anytime_eps0_share}{100\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps1_accuracy}{79.0\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{gate_eps1_escalation}{75.1\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{gate_eps1_share}{88\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps1_accuracy}{78.9\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_accuracy)
\tjset{anytime_eps1_share}{82\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps2_accuracy}{77.9\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_accuracy)
\tjset{gate_eps2_escalation}{65.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, 1 - test_coverage)
\tjset{gate_eps2_share}{80\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps2_accuracy}{78.0\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_accuracy)
\tjset{anytime_eps2_share}{73\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{stop_s1}{23.7\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered by S1
\tjset{stop_checkpoint}{22.9\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered at a checkpoint before the full thought
\tjset{stop_full}{53.4\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered after the full thought
\tjset{stop_checkpoint_of_escalated}{30.1\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of escalated rows that stop at a checkpoint
\tjset{lang_en_rows}{1445} % `per_family_test` (rows, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s1}{46.9\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s2}{98.8\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_system}{97.9\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_escalation}{89.1\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'en')
\tjset{lang_zh_rows}{947} % `per_family_test` (rows, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s1}{45.4\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s2}{98.4\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_system}{98.1\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_escalation}{93.7\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'zh')
\tjset{combined_eps0_accuracy}{80.0\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_accuracy)
\tjset{combined_eps0_escalation}{96.5\%} % `dev_selected_operating_points` (combined, tolerance 0.0, 1 - test_coverage)
\tjset{combined_eps0_share}{99\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps1_accuracy}{78.9\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_accuracy)
\tjset{combined_eps1_escalation}{74.4\%} % `dev_selected_operating_points` (combined, tolerance 0.01, 1 - test_coverage)
\tjset{combined_eps1_share}{88\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps2_accuracy}{77.7\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_accuracy)
\tjset{combined_eps2_escalation}{65.0\%} % `dev_selected_operating_points` (combined, tolerance 0.02, 1 - test_coverage)
\tjset{combined_eps2_share}{79\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_weight_confidence_rot}{1.042} % `combined_fit.standardized_weights.confidence_rot`
\tjset{combined_weight_router_zero_shot}{0.089} % `combined_fit.standardized_weights.router_zero_shot`
\tjset{auroc_confidence}{0.753} % `auroc_s1_correct_test.confidence`
\tjset{auroc_confidence_rot}{0.753} % `auroc_s1_correct_test.confidence_rot`
\tjset{auroc_probe}{0.796} % `auroc_s1_correct_test.probe`
\tjset{auroc_router_probe}{0.779} % `auroc_s1_correct_test.router_probe`
\tjset{auroc_router_zero_shot}{0.667} % `auroc_s1_correct_test.router_zero_shot`
\tjset{auroc_router_supervised}{0.670} % `auroc_s1_correct_test.router_supervised`
\tjset{auroc_combined}{0.752} % `auroc_s1_correct_test.combined`
\tjset{area_confidence}{0.367} % `normalized_area_test.area.confidence`
\tjset{area_confidence_rot}{0.367} % `normalized_area_test.area.confidence_rot`
\tjset{area_probe}{0.403} % `normalized_area_test.area.probe`
\tjset{area_router_probe}{0.381} % `normalized_area_test.area.router_probe`
\tjset{area_router_zero_shot}{0.430} % `normalized_area_test.area.router_zero_shot`
\tjset{area_router_supervised}{0.207} % `normalized_area_test.area.router_supervised`
\tjset{area_combined}{0.384} % `normalized_area_test.area.combined`
\tjset{area_diff_confidence}{$-$0.001} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_confidence}{[$-$0.021, +0.019]} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, ci95)
\tjset{area_diff_probe}{$-$0.037} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_probe}{[$-$0.062, $-$0.013]} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_probe}{$-$0.014} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_probe}{[$-$0.039, +0.009]} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_zero_shot}{$-$0.063} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_zero_shot}{[$-$0.091, $-$0.038]} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_supervised}{+0.159} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_supervised}{[+0.131, +0.189]} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, ci95)
\tjset{area_diff_combined}{$-$0.018} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_combined}{[$-$0.020, $-$0.015]} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, ci95)
\tjset{disagree_jev_fix}{350} % `disagreement_test.by_source` (summed over block 'jev', s1_wrong_s2_right)
\tjset{disagree_jev_break}{103} % `disagreement_test.by_source` (summed over block 'jev', s1_right_s2_wrong)
\tjset{disagree_public_fix}{738} % `disagreement_test.by_source` (summed over block 'public', s1_wrong_s2_right)
\tjset{disagree_public_break}{135} % `disagreement_test.by_source` (summed over block 'public', s1_right_s2_wrong)
\tjset{disagree_weak_fix}{1367} % `disagreement_test.by_source` (summed over block 'weak', s1_wrong_s2_right)
\tjset{disagree_weak_break}{54} % `disagreement_test.by_source` (summed over block 'weak', s1_right_s2_wrong)
\tjset{grp_arithmetic_rows}{288} % `per_family_test` (rows, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s1}{32.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_escalation}{100.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Arithmetic')
\tjset{grp_datecomparison_rows}{293} % `per_family_test` (rows, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s1}{34.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s2}{96.6\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_system}{96.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_escalation}{100.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date comparison')
\tjset{grp_chess_rows}{733} % `per_family_test` (rows, row-weighted over group 'Chess')
\tjset{grp_chess_s1}{37.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_s2}{42.3\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_system}{42.3\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_escalation}{99.2\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chess')
\tjset{grp_logicgrid_rows}{272} % `per_family_test` (rows, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s1}{44.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s2}{98.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_system}{98.5\%} % `per_family_test` (system_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_escalation}{99.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'Logic grid')
\tjset{grp_graphpaths_rows}{313} % `per_family_test` (rows, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s1}{47.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s2}{96.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_system}{95.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_escalation}{92.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Graph paths')
\tjset{grp_datedeadlines_rows}{27} % `per_family_test` (rows, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s1}{48.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_system}{74.1\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_escalation}{37.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date deadlines')
\tjset{grp_chainedrules_rows}{298} % `per_family_test` (rows, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s1}{48.7\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_system}{99.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_escalation}{92.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chained rules')
\tjset{grp_counting_rows}{345} % `per_family_test` (rows, row-weighted over group 'Counting')
\tjset{grp_counting_s1}{49.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_system}{99.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_escalation}{93.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Counting')
\tjset{grp_scheduling_rows}{301} % `per_family_test` (rows, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s1}{49.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s2}{99.3\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_system}{97.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_escalation}{84.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Scheduling')
\tjset{grp_stackednegation_rows}{315} % `per_family_test` (rows, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s1}{65.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s2}{98.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_system}{96.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_escalation}{68.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'Stacked negation')
\tjset{grp_doublenegationhard200_rows}{30} % `per_family_test` (rows, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s1}{86.7\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s2}{90.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_system}{90.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_escalation}{33.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Double negation (hard200)')
\tjset{grp_multihopruleshard200_rows}{31} % `per_family_test` (rows, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s1}{87.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_escalation}{74.2\%} % `per_family_test` (escalation_rate, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_escalationclinc_rows}{290} % `per_family_test` (rows, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s1}{53.4\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s2}{84.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_system}{72.1\%} % `per_family_test` (system_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_escalation}{36.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_typeddecisions_rows}{1165} % `per_family_test` (rows, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s1}{63.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s2}{71.8\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_system}{71.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_escalation}{66.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Typed decisions')
\tjset{grp_nliwanli_rows}{159} % `per_family_test` (rows, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s1}{67.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s2}{75.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_system}{74.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_escalation}{54.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'NLI (WANLI)')
\tjset{grp_intentroutingbanking77_rows}{486} % `per_family_test` (rows, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s1}{78.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s2}{82.9\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_system}{82.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_escalation}{31.5\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingclinc_rows}{358} % `per_family_test` (rows, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s1}{91.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s2}{97.8\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_system}{97.8\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_escalation}{27.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_semifauthored_rows}{84} % `per_family_test` (rows, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s1}{92.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s2}{94.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_system}{94.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_escalation}{32.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'SemIf authored')
\tjset{grp_everyjudgments_rows}{84} % `per_family_test` (rows, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s1}{94.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s2}{95.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_system}{95.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_escalation}{8.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Every judgments')
\tjset{grp_supergpqa_rows}{652} % `per_family_test` (rows, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s1}{35.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s2}{51.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_system}{51.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_escalation}{93.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'SuperGPQA')
\tjset{grp_mmlupro_rows}{715} % `per_family_test` (rows, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s1}{44.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s2}{76.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_system}{75.9\%} % `per_family_test` (system_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_escalation}{86.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'MMLU-Pro')
\tjset{grp_gpqadiamond_rows}{117} % `per_family_test` (rows, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s1}{46.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s2}{73.5\%} % `per_family_test` (s2_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_system}{73.5\%} % `per_family_test` (system_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_escalation}{94.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'GPQA Diamond')
\tjset{grp_musr_rows}{383} % `per_family_test` (rows, row-weighted over group 'MuSR')
\tjset{grp_musr_s1}{54.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_s2}{63.4\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_system}{61.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_escalation}{63.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'MuSR')
\tjset{grp_bigbenchhard_rows}{620} % `per_family_test` (rows, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s1}{59.4\%} % `per_family_test` (s1_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s2}{92.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_system}{92.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_escalation}{74.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'BIG-Bench Hard')
\tjset{difficulty_families}{9} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty computed per family)
\tjset{difficulty_rising}{7} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty > 0)
\tjset{weak_d1_rows}{767} % `per_family_test` (rows, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_escalation}{78.0\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s1}{58.7\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s2}{91.5\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d2_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_escalation}{95.3\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s1}{48.4\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s2}{85.6\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d3_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_escalation}{98.4\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s1}{35.9\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s2}{84.5\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d4_rows}{776} % `per_family_test` (rows, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_escalation}{99.5\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s1}{34.4\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s2}{80.2\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 4)
\tjset{jb_s1_correct}{190} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s1` (correct)
\tjset{jb_s1_acc}{82.3\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s1` (accuracy)
\tjset{jb_s1_hard_correct}{72} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s1` (by_tier.hard.correct)
\tjset{jb_s1_hard_acc}{64.9\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s1` (by_tier.hard.accuracy)
\tjset{jb_s1_ece}{0.043} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s1` (ece)
\tjset{jb_s1_think}{0} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s1` (mean_think_tokens)
\tjset{jb_s1_escalation}{0.0\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s1` (escalation_rate)
\tjset{jb_s1_vs_jev1130_all_ours}{9} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.jev-1.13.0.all` (ours_only)
\tjset{jb_s1_vs_jev1130_all_theirs}{19} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.jev-1.13.0.all` (theirs_only)
\tjset{jb_s1_vs_jev1130_all_p}{$p = 0.087$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.jev-1.13.0.all` (p_value)
\tjset{jb_s1_vs_jev1130_hard_ours}{8} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.jev-1.13.0.hard` (ours_only)
\tjset{jb_s1_vs_jev1130_hard_theirs}{17} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s1_vs_jev1130_hard_p}{$p = 0.108$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.jev-1.13.0.hard` (p_value)
\tjset{jb_s1_vs_openjevthinking_all_ours}{12} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.openjev-thinking.all` (ours_only)
\tjset{jb_s1_vs_openjevthinking_all_theirs}{27} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.openjev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_all_p}{$p = 0.024$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.openjev-thinking.all` (p_value)
\tjset{jb_s1_vs_openjevthinking_hard_ours}{12} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.openjev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_openjevthinking_hard_theirs}{25} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.openjev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_hard_p}{$p = 0.047$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.openjev-thinking.hard` (p_value)
\tjset{jb_s1_vs_djevthinking_all_ours}{20} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.djev-thinking.all` (ours_only)
\tjset{jb_s1_vs_djevthinking_all_theirs}{32} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.djev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_djevthinking_all_p}{$p = 0.126$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.djev-thinking.all` (p_value)
\tjset{jb_s1_vs_djevthinking_hard_ours}{17} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.djev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_djevthinking_hard_theirs}{30} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.djev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_djevthinking_hard_p}{$p = 0.079$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.djev-thinking.hard` (p_value)
\tjset{jb_s1_vs_semifqwen354b_all_ours}{19} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_all_theirs}{16} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_all_p}{$p = 0.736$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s1_vs_semifqwen354b_hard_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_hard_theirs}{14} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_hard_p}{$p = 0.597$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s1_vs_reflex27b_all_ours}{8} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.reflex-27b.all` (ours_only)
\tjset{jb_s1_vs_reflex27b_all_theirs}{19} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.reflex-27b.all` (theirs_only)
\tjset{jb_s1_vs_reflex27b_all_p}{$p = 0.052$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.reflex-27b.all` (p_value)
\tjset{jb_s1_vs_reflex27b_hard_ours}{5} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.reflex-27b.hard` (ours_only)
\tjset{jb_s1_vs_reflex27b_hard_theirs}{17} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.reflex-27b.hard` (theirs_only)
\tjset{jb_s1_vs_reflex27b_hard_p}{$p = 0.017$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.reflex-27b.hard` (p_value)
\tjset{jb_s1_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.deepseek-flash.all` (ours_only)
\tjset{jb_s1_vs_deepseekflash_all_theirs}{40} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.deepseek-flash.all` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.deepseek-flash.all` (p_value)
\tjset{jb_s1_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.deepseek-flash.hard` (ours_only)
\tjset{jb_s1_vs_deepseekflash_hard_theirs}{38} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.deepseek-flash.hard` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.deepseek-flash.hard` (p_value)
\tjset{jb_s1_vs_gpt56luna_all_ours}{2} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s1_vs_gpt56luna_all_theirs}{37} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (p_value)
\tjset{jb_s1_vs_gpt56luna_hard_ours}{0} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s1_vs_gpt56luna_hard_theirs}{35} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (p_value)
\tjset{jb_s2_correct}{219} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s2` (correct)
\tjset{jb_s2_acc}{94.8\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s2` (accuracy)
\tjset{jb_s2_hard_correct}{99} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s2` (by_tier.hard.correct)
\tjset{jb_s2_hard_acc}{89.2\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s2` (by_tier.hard.accuracy)
\tjset{jb_s2_ece}{0.072} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s2` (ece)
\tjset{jb_s2_think}{1472} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s2` (mean_think_tokens)
\tjset{jb_s2_escalation}{100.0\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.s2` (escalation_rate)
\tjset{jb_s2_vs_jev1130_all_ours}{23} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.jev-1.13.0.all` (ours_only)
\tjset{jb_s2_vs_jev1130_all_theirs}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.jev-1.13.0.all` (theirs_only)
\tjset{jb_s2_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.jev-1.13.0.all` (p_value)
\tjset{jb_s2_vs_jev1130_hard_ours}{22} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.jev-1.13.0.hard` (ours_only)
\tjset{jb_s2_vs_jev1130_hard_theirs}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s2_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.jev-1.13.0.hard` (p_value)
\tjset{jb_s2_vs_openjevthinking_all_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.openjev-thinking.all` (ours_only)
\tjset{jb_s2_vs_openjevthinking_all_theirs}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.openjev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_all_p}{$p = 0.004$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.openjev-thinking.all` (p_value)
\tjset{jb_s2_vs_openjevthinking_hard_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.openjev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_openjevthinking_hard_theirs}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.openjev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_hard_p}{$p = 0.004$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.openjev-thinking.hard` (p_value)
\tjset{jb_s2_vs_djevthinking_all_ours}{26} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.djev-thinking.all` (ours_only)
\tjset{jb_s2_vs_djevthinking_all_theirs}{9} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.djev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_djevthinking_all_p}{$p = 0.006$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.djev-thinking.all` (p_value)
\tjset{jb_s2_vs_djevthinking_hard_ours}{23} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.djev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_djevthinking_hard_theirs}{9} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.djev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_djevthinking_hard_p}{$p = 0.020$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.djev-thinking.hard` (p_value)
\tjset{jb_s2_vs_semifqwen354b_all_ours}{35} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_all_theirs}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s2_vs_semifqwen354b_hard_ours}{34} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_hard_theirs}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s2_vs_reflex27b_all_ours}{23} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.reflex-27b.all` (ours_only)
\tjset{jb_s2_vs_reflex27b_all_theirs}{5} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.reflex-27b.all` (theirs_only)
\tjset{jb_s2_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.reflex-27b.all` (p_value)
\tjset{jb_s2_vs_reflex27b_hard_ours}{20} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.reflex-27b.hard` (ours_only)
\tjset{jb_s2_vs_reflex27b_hard_theirs}{5} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.reflex-27b.hard` (theirs_only)
\tjset{jb_s2_vs_reflex27b_hard_p}{$p = 0.004$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.reflex-27b.hard` (p_value)
\tjset{jb_s2_vs_deepseekflash_all_ours}{5} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.deepseek-flash.all` (ours_only)
\tjset{jb_s2_vs_deepseekflash_all_theirs}{12} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.deepseek-flash.all` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_all_p}{$p = 0.143$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.deepseek-flash.all` (p_value)
\tjset{jb_s2_vs_deepseekflash_hard_ours}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.deepseek-flash.hard` (ours_only)
\tjset{jb_s2_vs_deepseekflash_hard_theirs}{12} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.deepseek-flash.hard` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_hard_p}{$p = 0.077$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.deepseek-flash.hard` (p_value)
\tjset{jb_s2_vs_gpt56luna_all_ours}{5} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s2_vs_gpt56luna_all_theirs}{11} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_all_p}{$p = 0.210$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (p_value)
\tjset{jb_s2_vs_gpt56luna_hard_ours}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s2_vs_gpt56luna_hard_theirs}{11} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_hard_p}{$p = 0.057$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (p_value)
\tjset{jb_gate_correct}{218} % `jevbench-qwen3.5-9b-report-v2.json` `policies.gate` (correct)
\tjset{jb_gate_acc}{94.4\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.gate` (accuracy)
\tjset{jb_gate_hard_correct}{98} % `jevbench-qwen3.5-9b-report-v2.json` `policies.gate` (by_tier.hard.correct)
\tjset{jb_gate_hard_acc}{88.3\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.gate` (by_tier.hard.accuracy)
\tjset{jb_gate_ece}{0.054} % `jevbench-qwen3.5-9b-report-v2.json` `policies.gate` (ece)
\tjset{jb_gate_think}{1026} % `jevbench-qwen3.5-9b-report-v2.json` `policies.gate` (mean_think_tokens)
\tjset{jb_gate_escalation}{42.0\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.gate` (escalation_rate)
\tjset{jb_gate_vs_jev1130_all_ours}{20} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.jev-1.13.0.all` (ours_only)
\tjset{jb_gate_vs_jev1130_all_theirs}{2} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.jev-1.13.0.all` (theirs_only)
\tjset{jb_gate_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.jev-1.13.0.all` (p_value)
\tjset{jb_gate_vs_jev1130_hard_ours}{19} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.jev-1.13.0.hard` (ours_only)
\tjset{jb_gate_vs_jev1130_hard_theirs}{2} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.jev-1.13.0.hard` (theirs_only)
\tjset{jb_gate_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.jev-1.13.0.hard` (p_value)
\tjset{jb_gate_vs_openjevthinking_all_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.openjev-thinking.all` (ours_only)
\tjset{jb_gate_vs_openjevthinking_all_theirs}{5} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.openjev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_all_p}{$p = 0.011$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.openjev-thinking.all` (p_value)
\tjset{jb_gate_vs_openjevthinking_hard_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.openjev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_openjevthinking_hard_theirs}{5} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.openjev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_hard_p}{$p = 0.011$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.openjev-thinking.hard` (p_value)
\tjset{jb_gate_vs_djevthinking_all_ours}{24} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.djev-thinking.all` (ours_only)
\tjset{jb_gate_vs_djevthinking_all_theirs}{8} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.djev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_djevthinking_all_p}{$p = 0.007$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.djev-thinking.all` (p_value)
\tjset{jb_gate_vs_djevthinking_hard_ours}{21} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.djev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_djevthinking_hard_theirs}{8} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.djev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_djevthinking_hard_p}{$p = 0.024$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.djev-thinking.hard` (p_value)
\tjset{jb_gate_vs_semifqwen354b_all_ours}{33} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_all_theirs}{2} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_gate_vs_semifqwen354b_hard_ours}{32} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_hard_theirs}{2} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_gate_vs_reflex27b_all_ours}{20} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.reflex-27b.all` (ours_only)
\tjset{jb_gate_vs_reflex27b_all_theirs}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.reflex-27b.all` (theirs_only)
\tjset{jb_gate_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.reflex-27b.all` (p_value)
\tjset{jb_gate_vs_reflex27b_hard_ours}{17} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.reflex-27b.hard` (ours_only)
\tjset{jb_gate_vs_reflex27b_hard_theirs}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.reflex-27b.hard` (theirs_only)
\tjset{jb_gate_vs_reflex27b_hard_p}{$p = 0.003$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.reflex-27b.hard` (p_value)
\tjset{jb_gate_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.deepseek-flash.all` (ours_only)
\tjset{jb_gate_vs_deepseekflash_all_theirs}{12} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.deepseek-flash.all` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_all_p}{$p = 0.077$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.deepseek-flash.all` (p_value)
\tjset{jb_gate_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.deepseek-flash.hard` (ours_only)
\tjset{jb_gate_vs_deepseekflash_hard_theirs}{12} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.deepseek-flash.hard` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_hard_p}{$p = 0.035$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.deepseek-flash.hard` (p_value)
\tjset{jb_gate_vs_gpt56luna_all_ours}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (ours_only)
\tjset{jb_gate_vs_gpt56luna_all_theirs}{10} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_all_p}{$p = 0.092$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (p_value)
\tjset{jb_gate_vs_gpt56luna_hard_ours}{1} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_gate_vs_gpt56luna_hard_theirs}{10} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_hard_p}{$p = 0.012$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (p_value)
\tjset{jb_anytime_correct}{216} % `jevbench-qwen3.5-9b-report-v2.json` `policies.anytime` (correct)
\tjset{jb_anytime_acc}{93.5\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.anytime` (accuracy)
\tjset{jb_anytime_hard_correct}{97} % `jevbench-qwen3.5-9b-report-v2.json` `policies.anytime` (by_tier.hard.correct)
\tjset{jb_anytime_hard_acc}{87.4\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.anytime` (by_tier.hard.accuracy)
\tjset{jb_anytime_ece}{0.050} % `jevbench-qwen3.5-9b-report-v2.json` `policies.anytime` (ece)
\tjset{jb_anytime_think}{929} % `jevbench-qwen3.5-9b-report-v2.json` `policies.anytime` (mean_think_tokens)
\tjset{jb_anytime_escalation}{42.0\%} % `jevbench-qwen3.5-9b-report-v2.json` `policies.anytime` (escalation_rate)
\tjset{jb_anytime_vs_jev1130_all_ours}{19} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.jev-1.13.0.all` (ours_only)
\tjset{jb_anytime_vs_jev1130_all_theirs}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.jev-1.13.0.all` (theirs_only)
\tjset{jb_anytime_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.jev-1.13.0.all` (p_value)
\tjset{jb_anytime_vs_jev1130_hard_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (ours_only)
\tjset{jb_anytime_vs_jev1130_hard_theirs}{2} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (theirs_only)
\tjset{jb_anytime_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (p_value)
\tjset{jb_anytime_vs_openjevthinking_all_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.openjev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_all_theirs}{7} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.openjev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_all_p}{$p = 0.043$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.openjev-thinking.all` (p_value)
\tjset{jb_anytime_vs_openjevthinking_hard_ours}{18} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.openjev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_hard_theirs}{6} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.openjev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_hard_p}{$p = 0.023$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.openjev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_djevthinking_all_ours}{24} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.djev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_djevthinking_all_theirs}{10} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.djev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_all_p}{$p = 0.024$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.djev-thinking.all` (p_value)
\tjset{jb_anytime_vs_djevthinking_hard_ours}{21} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.djev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_djevthinking_hard_theirs}{9} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.djev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_hard_p}{$p = 0.043$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.djev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_all_ours}{33} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_all_theirs}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_hard_ours}{32} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_theirs}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_anytime_vs_reflex27b_all_ours}{19} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.reflex-27b.all` (ours_only)
\tjset{jb_anytime_vs_reflex27b_all_theirs}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.reflex-27b.all` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_all_p}{$p = 0.003$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.reflex-27b.all` (p_value)
\tjset{jb_anytime_vs_reflex27b_hard_ours}{16} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.reflex-27b.hard` (ours_only)
\tjset{jb_anytime_vs_reflex27b_hard_theirs}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.reflex-27b.hard` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_hard_p}{$p = 0.004$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.reflex-27b.hard` (p_value)
\tjset{jb_anytime_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.deepseek-flash.all` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_all_theirs}{14} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.deepseek-flash.all` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_all_p}{$p = 0.031$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.deepseek-flash.all` (p_value)
\tjset{jb_anytime_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.deepseek-flash.hard` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_hard_theirs}{13} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.deepseek-flash.hard` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_hard_p}{$p = 0.021$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.deepseek-flash.hard` (p_value)
\tjset{jb_anytime_vs_gpt56luna_all_ours}{3} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_all_theirs}{12} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_all_p}{$p = 0.035$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (p_value)
\tjset{jb_anytime_vs_gpt56luna_hard_ours}{1} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_hard_theirs}{11} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_hard_p}{$p = 0.006$} % `jevbench-qwen3.5-9b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (p_value)
\tjset{jb_sys_jev1130_correct}{200} % `jevbench-qwen3.5-9b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (correct)
\tjset{jb_sys_jev1130_acc}{86.6\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_jev1130_hard_correct}{81} % `jevbench-qwen3.5-9b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_jev1130_hard_acc}{73.0\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_openjevthinking_correct}{205} % `jevbench-qwen3.5-9b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_openjevthinking_acc}{88.7\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_openjevthinking_hard_correct}{85} % `jevbench-qwen3.5-9b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_openjevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_djevthinking_correct}{202} % `jevbench-qwen3.5-9b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_djevthinking_acc}{87.4\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_djevthinking_hard_correct}{85} % `jevbench-qwen3.5-9b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_djevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_semifqwen354b_correct}{187} % `jevbench-qwen3.5-9b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (correct)
\tjset{jb_sys_semifqwen354b_acc}{81.0\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_semifqwen354b_hard_correct}{68} % `jevbench-qwen3.5-9b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_semifqwen354b_hard_acc}{61.3\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_reflex27b_correct}{201} % `jevbench-qwen3.5-9b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (correct)
\tjset{jb_sys_reflex27b_acc}{87.0\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_reflex27b_hard_correct}{84} % `jevbench-qwen3.5-9b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_reflex27b_hard_acc}{75.7\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_deepseekflash_correct}{226} % `jevbench-qwen3.5-9b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (correct)
\tjset{jb_sys_deepseekflash_acc}{97.8\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_deepseekflash_hard_correct}{107} % `jevbench-qwen3.5-9b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_deepseekflash_hard_acc}{96.4\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_gpt56luna_correct}{225} % `jevbench-qwen3.5-9b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (correct)
\tjset{jb_sys_gpt56luna_acc}{97.4\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_gpt56luna_hard_correct}{107} % `jevbench-qwen3.5-9b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_gpt56luna_hard_acc}{96.4\%} % `jevbench-qwen3.5-9b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_rows}{231} % `jevbench-qwen3.5-9b-report-v2.json` `policies.*.n`
\tjset{jb_hard_rows}{111} % `jevbench-qwen3.5-9b-report-v2.json` `policies.*.by_tier.hard.n`


==> figures/qwen3.5-9b/per_source.tex <==
A & Escalation (CLINC) & en & -- & 290 & 53.4\% & 84.1\% & 72.1\% & 36.6\% \\
A & Every judgments & en & -- & 84 & 94.0\% & 95.2\% & 95.2\% & 8.3\% \\
A & Intent routing (BANKING77) & en & -- & 486 & 78.6\% & 82.9\% & 82.7\% & 31.5\% \\
A & Intent routing (CLINC) & en & -- & 358 & 91.3\% & 97.8\% & 97.8\% & 27.4\% \\
A & NLI (WANLI) & en & -- & 159 & 67.3\% & 75.5\% & 74.8\% & 54.7\% \\
A & SemIf authored & en & -- & 84 & 92.9\% & 94.0\% & 94.0\% & 32.1\% \\
A & Typed decisions & en & -- & 1165 & 63.3\% & 71.8\% & 71.0\% & 66.4\% \\
\midrule
B & BIG-Bench Hard & en & -- & 620 & 59.4\% & 92.7\% & 92.6\% & 74.7\% \\
B & GPQA Diamond & en & -- & 117 & 46.2\% & 73.5\% & 73.5\% & 94.0\% \\
B & MMLU-Pro & en & -- & 715 & 44.5\% & 76.2\% & 75.9\% & 86.7\% \\
B & MuSR & en & -- & 383 & 54.8\% & 63.4\% & 61.6\% & 63.4\% \\
B & SuperGPQA & en & -- & 652 & 35.6\% & 51.5\% & 51.2\% & 93.7\% \\
\midrule
C & Chess (Lichess) & en & 1 & 121 & 57.0\% & 66.1\% & 66.1\% & 97.5\% \\
C & Chess (Lichess) & en & 2 & 125 & 34.4\% & 40.0\% & 40.0\% & 99.2\% \\
C & Chess (Lichess) & en & 3 & 126 & 30.2\% & 35.7\% & 35.7\% & 100.0\% \\
C & Chess (Lichess) & en & 4 & 122 & 31.1\% & 32.0\% & 32.0\% & 100.0\% \\
C & Chess (Lichess) & zh & 1 & 58 & 58.6\% & 60.3\% & 60.3\% & 96.6\% \\
C & Chess (Lichess) & zh & 2 & 59 & 35.6\% & 40.7\% & 40.7\% & 100.0\% \\
C & Chess (Lichess) & zh & 3 & 60 & 33.3\% & 35.0\% & 35.0\% & 100.0\% \\
C & Chess (Lichess) & zh & 4 & 62 & 22.6\% & 25.8\% & 25.8\% & 100.0\% \\
C & Generated families & en & 1 & 356 & 57.6\% & 99.7\% & 98.0\% & 68.3\% \\
C & Generated families & en & 2 & 362 & 54.7\% & 98.9\% & 97.8\% & 91.7\% \\
C & Generated families & en & 3 & 358 & 39.1\% & 100.0\% & 99.4\% & 97.2\% \\
C & Generated families & en & 4 & 369 & 36.3\% & 96.5\% & 96.2\% & 98.9\% \\
C & Generated families & zh & 1 & 232 & 61.2\% & 100.0\% & 98.7\% & 78.0\% \\
C & Generated families & zh & 2 & 245 & 49.4\% & 100.0\% & 100.0\% & 97.6\% \\
C & Generated families & zh & 3 & 247 & 34.8\% & 98.8\% & 98.8\% & 98.8\% \\
C & Generated families & zh & 4 & 223 & 36.3\% & 94.6\% & 94.6\% & 100.0\% \\
C & hard200 fixture & en & -- & 121 & 74.4\% & 97.5\% & 91.7\% & 62.8\% \\


==> figures/qwen3.8-27b/data.tex <==
A & Escalation (CLINC) & 210 & 290 & en & CC-BY-3.0 \\
A & Every judgments & 70 & 84 & en & unstated \\
A & Intent routing (BANKING77) & 313 & 486 & en & CC-BY-4.0 \\
A & Intent routing (CLINC) & 242 & 358 & en & CC-BY-3.0 \\
A & NLI (WANLI) & 97 & 159 & en & CC-BY-4.0 \\
A & SemIf authored & 60 & 84 & en & MIT \\
A & Typed decisions & 835 & 1165 & en & Apache-2.0 \\
\midrule
B & BIG-Bench Hard & 400 & 620 & en & MIT \\
B & GPQA Diamond & 81 & 117 & en & CC-BY-4.0 \\
B & MMLU-Pro & 475 & 715 & en & MIT \\
B & MuSR & 217 & 383 & en & CC-BY-4.0 \\
B & SuperGPQA & 428 & 652 & en & ODC-BY-1.0 \\
\midrule
C & Chess (Lichess) & 467 & 733 & en, zh & CC0-1.0 \\
C & Generated families & 1608 & 2392 & en, zh & MIT \\
C & hard200 fixture & 79 & 121 & en & MIT \\
\midrule
All & & 5582 & 8359 & & \\


==> figures/qwen3.8-27b/numbers.tex <==
\tjset{rows_test}{8359} % `rows.test`
\tjset{always_s1_accuracy}{60.2\%} % `baselines_test.always_s1_accuracy`
\tjset{always_s2_accuracy}{81.8\%} % `baselines_test.always_s2_accuracy`
\tjset{always_s2_mean_think_tokens}{722} % `baselines_test.s2_mean_think_tokens`
\tjset{s1_wrong_s2_right}{2172} % `baselines_test.s1_wrong_s2_right`
\tjset{s1_right_s2_wrong}{367} % `baselines_test.s1_right_s2_wrong`
\tjset{s1_ece}{0.029} % `s1_readouts_test.*.ece`
\tjset{gate_test_accuracy}{80.9\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_mean_think_tokens}{619} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01)
\tjset{gate_thinking_share}{86\%} % `anytime_test.dev_selected_operating_points` (gate, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{anytime_test_accuracy}{80.8\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_mean_think_tokens}{612} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01)
\tjset{anytime_thinking_share}{85\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01) / `baselines_test.s2_mean_think_tokens`
\tjset{s1_ltt_coverage_at_5pct}{23.2\%} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_5pct}{4.2\%} % `s1_readouts_test.*.coverage_at_risk` (risk 0.05, ltt_test_risk)
\tjset{block_all_rows}{8359} % `per_family_test` (rows, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s1}{60.2\%} % `per_family_test` (s1_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_s2}{81.8\%} % `per_family_test` (s2_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_system}{80.8\%} % `per_family_test` (system_accuracy, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_all_escalation}{60.6\%} % `per_family_test` (escalation_rate, row-weighted over block 'all', gate `per_family_test_gate`)
\tjset{block_jev_rows}{2626} % `per_family_test` (rows, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s1}{78.9\%} % `per_family_test` (s1_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_s2}{81.7\%} % `per_family_test` (s2_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_system}{81.9\%} % `per_family_test` (system_accuracy, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_jev_escalation}{36.6\%} % `per_family_test` (escalation_rate, row-weighted over block 'jev', gate `per_family_test_gate`)
\tjset{block_public_rows}{2487} % `per_family_test` (rows, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s1}{54.5\%} % `per_family_test` (s1_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_s2}{73.9\%} % `per_family_test` (s2_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_system}{73.7\%} % `per_family_test` (system_accuracy, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_public_escalation}{64.7\%} % `per_family_test` (escalation_rate, row-weighted over block 'public', gate `per_family_test_gate`)
\tjset{block_weak_rows}{3246} % `per_family_test` (rows, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s1}{49.5\%} % `per_family_test` (s1_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_s2}{87.9\%} % `per_family_test` (s2_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_system}{85.3\%} % `per_family_test` (system_accuracy, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{block_weak_escalation}{76.9\%} % `per_family_test` (escalation_rate, row-weighted over block 'weak', gate `per_family_test_gate`)
\tjset{oracle_accuracy}{86.2\%} % `baselines_test.oracle_best_accuracy`
\tjset{s2_closed_naturally}{95.2\%} % `baselines_test.s2_closed_naturally_rate`
\tjset{disagree_total}{2539} % `baselines_test.s1_wrong_s2_right` + `s1_right_s2_wrong`
\tjset{h2_accuracy}{80.8\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{h2_gap}{1.0} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, always-S2 accuracy minus test_accuracy, in points)
\tjset{h2_escalation}{60.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{s1_raw_accuracy}{60.2\%} % `s1_readouts_test.raw.accuracy`
\tjset{s1_raw_ece}{0.017} % `s1_readouts_test.raw.ece`
\tjset{s1_rotation_accuracy}{62.8\%} % `s1_readouts_test.rotation.accuracy`
\tjset{s1_rotation_ece}{0.029} % `s1_readouts_test.rotation.ece`
\tjset{s1_ece_uncalibrated}{0.045} % `s1_readouts_test.rotation.ece_t1`
\tjset{s1_prior_accuracy}{61.5\%} % `s1_readouts_test.rotation_batch_prior.accuracy`
\tjset{s1_prior_ece}{0.074} % `s1_readouts_test.rotation_batch_prior.ece`
\tjset{s1_order_flip_rate}{44.5\%} % `order_flip_rate_test.all`
\tjset{temp_s1}{1.18} % `s1_readouts_test.rotation.temperature`
\tjset{s1_ltt_coverage_at_1pct}{6.9\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_1pct}{0.5\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, ltt_test_risk)
\tjset{s1_ltt_interval_at_1pct}{[0.1, 1.5]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.01, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_2pct}{10.5\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_2pct}{1.0\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, ltt_test_risk)
\tjset{s1_ltt_interval_at_2pct}{[0.5, 1.9]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.02, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_interval_at_5pct}{[3.3, 5.2]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.05, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_coverage_at_10pct}{37.6\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_coverage)
\tjset{s1_ltt_test_risk_at_10pct}{10.5\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, ltt_test_risk)
\tjset{s1_ltt_interval_at_10pct}{[9.5, 11.7]\%} % `s1_readouts_test.rotation.coverage_at_risk` (risk 0.1, exact binomial 95% interval of ltt_test_risk over ltt_test_coverage x rows.test)
\tjset{s1_ltt_targets_certified}{4} % `s1_readouts_test.rotation.coverage_at_risk` (targets with ltt_test_coverage > 0)
\tjset{anytime_acc_t0}{59.9\%} % `anytime_test.per_checkpoint` (t = 0, accuracy)
\tjset{anytime_ece_t0}{0.029} % `anytime_test.per_checkpoint` (t = 0, ece)
\tjset{anytime_tokens_t0}{0} % `anytime_test.per_checkpoint` (t = 0, mean_think_tokens)
\tjset{anytime_acc_t128}{63.3\%} % `anytime_test.per_checkpoint` (t = 128, accuracy)
\tjset{anytime_ece_t128}{0.025} % `anytime_test.per_checkpoint` (t = 128, ece)
\tjset{anytime_tokens_t128}{122} % `anytime_test.per_checkpoint` (t = 128, mean_think_tokens)
\tjset{anytime_acc_t256}{69.5\%} % `anytime_test.per_checkpoint` (t = 256, accuracy)
\tjset{anytime_ece_t256}{0.048} % `anytime_test.per_checkpoint` (t = 256, ece)
\tjset{anytime_tokens_t256}{216} % `anytime_test.per_checkpoint` (t = 256, mean_think_tokens)
\tjset{anytime_acc_t512}{75.4\%} % `anytime_test.per_checkpoint` (t = 512, accuracy)
\tjset{anytime_ece_t512}{0.040} % `anytime_test.per_checkpoint` (t = 512, ece)
\tjset{anytime_tokens_t512}{338} % `anytime_test.per_checkpoint` (t = 512, mean_think_tokens)
\tjset{anytime_acc_t1024}{79.7\%} % `anytime_test.per_checkpoint` (t = 1024, accuracy)
\tjset{anytime_ece_t1024}{0.054} % `anytime_test.per_checkpoint` (t = 1024, ece)
\tjset{anytime_tokens_t1024}{462} % `anytime_test.per_checkpoint` (t = 1024, mean_think_tokens)
\tjset{anytime_acc_t2048}{81.4\%} % `anytime_test.per_checkpoint` (t = 2048, accuracy)
\tjset{anytime_ece_t2048}{0.052} % `anytime_test.per_checkpoint` (t = 2048, ece)
\tjset{anytime_tokens_t2048}{583} % `anytime_test.per_checkpoint` (t = 2048, mean_think_tokens)
\tjset{anytime_acc_full}{81.8\%} % `anytime_test.full_thought.accuracy`
\tjset{anytime_ece_full}{0.058} % `anytime_test.full_thought.ece`
\tjset{temp_t0}{1.68} % `anytime_test.per_checkpoint` (t = 0, temperature)
\tjset{temp_t128}{2.34} % `anytime_test.per_checkpoint` (t = 128, temperature)
\tjset{temp_t256}{3.16} % `anytime_test.per_checkpoint` (t = 256, temperature)
\tjset{temp_t512}{4.38} % `anytime_test.per_checkpoint` (t = 512, temperature)
\tjset{temp_t1024}{4.96} % `anytime_test.per_checkpoint` (t = 1024, temperature)
\tjset{temp_t2048}{5.14} % `anytime_test.per_checkpoint` (t = 2048, temperature)
\tjset{temp_full}{5.31} % `anytime_test.full_thought.temperature`
\tjset{gate_eps0_accuracy}{81.8\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_accuracy)
\tjset{gate_eps0_escalation}{81.9\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, 1 - test_coverage)
\tjset{gate_eps0_share}{96\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps0_accuracy}{81.8\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_accuracy)
\tjset{anytime_eps0_share}{97\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps1_accuracy}{80.8\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_accuracy)
\tjset{gate_eps1_escalation}{60.6\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, 1 - test_coverage)
\tjset{gate_eps1_share}{84\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps1_accuracy}{80.8\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_accuracy)
\tjset{anytime_eps1_share}{85\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{gate_eps2_accuracy}{79.7\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_accuracy)
\tjset{gate_eps2_escalation}{52.8\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, 1 - test_coverage)
\tjset{gate_eps2_share}{78\%} % `dev_selected_operating_points` (confidence_rot, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{anytime_eps2_accuracy}{79.9\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_accuracy)
\tjset{anytime_eps2_share}{76\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{stop_s1}{33.8\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered by S1
\tjset{stop_checkpoint}{8.3\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered at a checkpoint before the full thought
\tjset{stop_full}{57.9\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of test rows answered after the full thought
\tjset{stop_checkpoint_of_escalated}{12.5\%} % `anytime_test.dev_selected_operating_points` (anytime, tolerance 0.01, tau) replayed on `inputs.cascade` with `anytime_test.per_checkpoint` temperatures: share of escalated rows that stop at a checkpoint
\tjset{lang_en_rows}{1445} % `per_family_test` (rows, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s1}{51.7\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_s2}{99.1\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_system}{95.4\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'en')
\tjset{lang_en_escalation}{72.2\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'en')
\tjset{lang_zh_rows}{947} % `per_family_test` (rows, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s1}{52.2\%} % `per_family_test` (s1_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_s2}{99.5\%} % `per_family_test` (s2_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_system}{96.3\%} % `per_family_test` (system_accuracy, row-weighted over source 'owned', lang 'zh')
\tjset{lang_zh_escalation}{75.6\%} % `per_family_test` (escalation_rate, row-weighted over source 'owned', lang 'zh')
\tjset{combined_eps0_accuracy}{81.7\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_accuracy)
\tjset{combined_eps0_escalation}{81.6\%} % `dev_selected_operating_points` (combined, tolerance 0.0, 1 - test_coverage)
\tjset{combined_eps0_share}{96\%} % `dev_selected_operating_points` (combined, tolerance 0.0, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps1_accuracy}{80.6\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_accuracy)
\tjset{combined_eps1_escalation}{56.6\%} % `dev_selected_operating_points` (combined, tolerance 0.01, 1 - test_coverage)
\tjset{combined_eps1_share}{82\%} % `dev_selected_operating_points` (combined, tolerance 0.01, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_eps2_accuracy}{79.5\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_accuracy)
\tjset{combined_eps2_escalation}{48.9\%} % `dev_selected_operating_points` (combined, tolerance 0.02, 1 - test_coverage)
\tjset{combined_eps2_share}{76\%} % `dev_selected_operating_points` (combined, tolerance 0.02, test_mean_think_tokens / `baselines_test.s2_mean_think_tokens`)
\tjset{combined_weight_confidence_rot}{1.468} % `combined_fit.standardized_weights.confidence_rot`
\tjset{combined_weight_router_zero_shot}{0.155} % `combined_fit.standardized_weights.router_zero_shot`
\tjset{auroc_confidence}{0.805} % `auroc_s1_correct_test.confidence`
\tjset{auroc_confidence_rot}{0.798} % `auroc_s1_correct_test.confidence_rot`
\tjset{auroc_probe}{0.771} % `auroc_s1_correct_test.probe`
\tjset{auroc_router_probe}{0.767} % `auroc_s1_correct_test.router_probe`
\tjset{auroc_router_zero_shot}{0.708} % `auroc_s1_correct_test.router_zero_shot`
\tjset{auroc_router_supervised}{0.706} % `auroc_s1_correct_test.router_supervised`
\tjset{auroc_combined}{0.798} % `auroc_s1_correct_test.combined`
\tjset{area_confidence}{0.425} % `normalized_area_test.area.confidence`
\tjset{area_confidence_rot}{0.421} % `normalized_area_test.area.confidence_rot`
\tjset{area_probe}{0.404} % `normalized_area_test.area.probe`
\tjset{area_router_probe}{0.400} % `normalized_area_test.area.router_probe`
\tjset{area_router_zero_shot}{0.488} % `normalized_area_test.area.router_zero_shot`
\tjset{area_router_supervised}{0.312} % `normalized_area_test.area.router_supervised`
\tjset{area_combined}{0.450} % `normalized_area_test.area.combined`
\tjset{area_diff_confidence}{$-$0.004} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_confidence}{[$-$0.024, +0.019]} % `normalized_area_test.difference_vs_primary.confidence` (confidence_rot minus policy, ci95)
\tjset{area_diff_probe}{+0.018} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_probe}{[$-$0.009, +0.045]} % `normalized_area_test.difference_vs_primary.probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_probe}{+0.021} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_probe}{[$-$0.005, +0.050]} % `normalized_area_test.difference_vs_primary.router_probe` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_zero_shot}{$-$0.067} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_zero_shot}{[$-$0.092, $-$0.041]} % `normalized_area_test.difference_vs_primary.router_zero_shot` (confidence_rot minus policy, ci95)
\tjset{area_diff_router_supervised}{+0.110} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_router_supervised}{[+0.080, +0.141]} % `normalized_area_test.difference_vs_primary.router_supervised` (confidence_rot minus policy, ci95)
\tjset{area_diff_combined}{$-$0.029} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, primary_minus_policy)
\tjset{area_ci_combined}{[$-$0.032, $-$0.025]} % `normalized_area_test.difference_vs_primary.combined` (confidence_rot minus policy, ci95)
\tjset{disagree_jev_fix}{212} % `disagreement_test.by_source` (summed over block 'jev', s1_wrong_s2_right)
\tjset{disagree_jev_break}{138} % `disagreement_test.by_source` (summed over block 'jev', s1_right_s2_wrong)
\tjset{disagree_public_fix}{617} % `disagreement_test.by_source` (summed over block 'public', s1_wrong_s2_right)
\tjset{disagree_public_break}{134} % `disagreement_test.by_source` (summed over block 'public', s1_right_s2_wrong)
\tjset{disagree_weak_fix}{1343} % `disagreement_test.by_source` (summed over block 'weak', s1_wrong_s2_right)
\tjset{disagree_weak_break}{95} % `disagreement_test.by_source` (summed over block 'weak', s1_right_s2_wrong)
\tjset{grp_datecomparison_rows}{293} % `per_family_test` (rows, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s1}{32.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_s2}{95.6\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_system}{95.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date comparison')
\tjset{grp_datecomparison_escalation}{100.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date comparison')
\tjset{grp_chess_rows}{733} % `per_family_test` (rows, row-weighted over group 'Chess')
\tjset{grp_chess_s1}{36.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_s2}{49.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_system}{49.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chess')
\tjset{grp_chess_escalation}{93.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chess')
\tjset{grp_arithmetic_rows}{288} % `per_family_test` (rows, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s1}{37.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_system}{98.3\%} % `per_family_test` (system_accuracy, row-weighted over group 'Arithmetic')
\tjset{grp_arithmetic_escalation}{97.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'Arithmetic')
\tjset{grp_logicgrid_rows}{272} % `per_family_test` (rows, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s1}{47.1\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_s2}{99.6\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_system}{98.5\%} % `per_family_test` (system_accuracy, row-weighted over group 'Logic grid')
\tjset{grp_logicgrid_escalation}{90.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'Logic grid')
\tjset{grp_graphpaths_rows}{313} % `per_family_test` (rows, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s1}{47.9\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_s2}{99.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_system}{90.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'Graph paths')
\tjset{grp_graphpaths_escalation}{61.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Graph paths')
\tjset{grp_chainedrules_rows}{298} % `per_family_test` (rows, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s1}{51.7\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_system}{85.9\%} % `per_family_test` (system_accuracy, row-weighted over group 'Chained rules')
\tjset{grp_chainedrules_escalation}{51.3\%} % `per_family_test` (escalation_rate, row-weighted over group 'Chained rules')
\tjset{grp_counting_rows}{345} % `per_family_test` (rows, row-weighted over group 'Counting')
\tjset{grp_counting_s1}{58.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_system}{99.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'Counting')
\tjset{grp_counting_escalation}{71.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Counting')
\tjset{grp_scheduling_rows}{301} % `per_family_test` (rows, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s1}{63.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Scheduling')
\tjset{grp_scheduling_escalation}{75.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Scheduling')
\tjset{grp_datedeadlines_rows}{27} % `per_family_test` (rows, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s1}{70.4\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_system}{92.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'Date deadlines')
\tjset{grp_datedeadlines_escalation}{70.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Date deadlines')
\tjset{grp_multihopruleshard200_rows}{31} % `per_family_test` (rows, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s1}{74.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_system}{80.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_multihopruleshard200_escalation}{19.4\%} % `per_family_test` (escalation_rate, row-weighted over group 'Multi-hop rules (hard200)')
\tjset{grp_stackednegation_rows}{315} % `per_family_test` (rows, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s1}{75.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_s2}{99.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_system}{98.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'Stacked negation')
\tjset{grp_stackednegation_escalation}{45.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Stacked negation')
\tjset{grp_doublenegationhard200_rows}{30} % `per_family_test` (rows, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s1}{100.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_s2}{100.0\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_system}{100.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Double negation (hard200)')
\tjset{grp_doublenegationhard200_escalation}{10.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'Double negation (hard200)')
\tjset{grp_escalationclinc_rows}{290} % `per_family_test` (rows, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s1}{65.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_s2}{80.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_system}{80.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_escalationclinc_escalation}{44.5\%} % `per_family_test` (escalation_rate, row-weighted over group 'Escalation (CLINC)')
\tjset{grp_typeddecisions_rows}{1165} % `per_family_test` (rows, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s1}{72.8\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_s2}{73.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_system}{74.0\%} % `per_family_test` (system_accuracy, row-weighted over group 'Typed decisions')
\tjset{grp_typeddecisions_escalation}{57.9\%} % `per_family_test` (escalation_rate, row-weighted over group 'Typed decisions')
\tjset{grp_nliwanli_rows}{159} % `per_family_test` (rows, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s1}{74.2\%} % `per_family_test` (s1_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_s2}{77.4\%} % `per_family_test` (s2_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_system}{76.7\%} % `per_family_test` (system_accuracy, row-weighted over group 'NLI (WANLI)')
\tjset{grp_nliwanli_escalation}{24.5\%} % `per_family_test` (escalation_rate, row-weighted over group 'NLI (WANLI)')
\tjset{grp_intentroutingbanking77_rows}{486} % `per_family_test` (rows, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s1}{85.6\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_s2}{87.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_system}{87.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_intentroutingbanking77_escalation}{14.2\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (BANKING77)')
\tjset{grp_semifauthored_rows}{84} % `per_family_test` (rows, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s1}{94.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_s2}{97.6\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_system}{97.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'SemIf authored')
\tjset{grp_semifauthored_escalation}{13.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'SemIf authored')
\tjset{grp_intentroutingclinc_rows}{358} % `per_family_test` (rows, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s1}{95.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_s2}{96.9\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_system}{96.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_intentroutingclinc_escalation}{8.7\%} % `per_family_test` (escalation_rate, row-weighted over group 'Intent routing (CLINC)')
\tjset{grp_everyjudgments_rows}{84} % `per_family_test` (rows, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s1}{96.4\%} % `per_family_test` (s1_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_s2}{97.6\%} % `per_family_test` (s2_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_system}{97.6\%} % `per_family_test` (system_accuracy, row-weighted over group 'Every judgments')
\tjset{grp_everyjudgments_escalation}{7.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'Every judgments')
\tjset{grp_supergpqa_rows}{652} % `per_family_test` (rows, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s1}{42.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_s2}{53.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_system}{54.4\%} % `per_family_test` (system_accuracy, row-weighted over group 'SuperGPQA')
\tjset{grp_supergpqa_escalation}{79.0\%} % `per_family_test` (escalation_rate, row-weighted over group 'SuperGPQA')
\tjset{grp_gpqadiamond_rows}{117} % `per_family_test` (rows, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s1}{48.7\%} % `per_family_test` (s1_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_s2}{75.2\%} % `per_family_test` (s2_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_system}{75.2\%} % `per_family_test` (system_accuracy, row-weighted over group 'GPQA Diamond')
\tjset{grp_gpqadiamond_escalation}{83.8\%} % `per_family_test` (escalation_rate, row-weighted over group 'GPQA Diamond')
\tjset{grp_mmlupro_rows}{715} % `per_family_test` (rows, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s1}{51.3\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_s2}{78.7\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_system}{78.3\%} % `per_family_test` (system_accuracy, row-weighted over group 'MMLU-Pro')
\tjset{grp_mmlupro_escalation}{67.1\%} % `per_family_test` (escalation_rate, row-weighted over group 'MMLU-Pro')
\tjset{grp_musr_rows}{383} % `per_family_test` (rows, row-weighted over group 'MuSR')
\tjset{grp_musr_s1}{59.0\%} % `per_family_test` (s1_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_s2}{67.9\%} % `per_family_test` (s2_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_system}{66.1\%} % `per_family_test` (system_accuracy, row-weighted over group 'MuSR')
\tjset{grp_musr_escalation}{43.6\%} % `per_family_test` (escalation_rate, row-weighted over group 'MuSR')
\tjset{grp_bigbenchhard_rows}{620} % `per_family_test` (rows, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s1}{69.5\%} % `per_family_test` (s1_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_s2}{93.1\%} % `per_family_test` (s2_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_system}{92.9\%} % `per_family_test` (system_accuracy, row-weighted over group 'BIG-Bench Hard')
\tjset{grp_bigbenchhard_escalation}{56.5\%} % `per_family_test` (escalation_rate, row-weighted over group 'BIG-Bench Hard')
\tjset{difficulty_families}{9} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty computed per family)
\tjset{difficulty_rising}{7} % `per_family_test` (owned families, rank correlation of escalation_rate with difficulty > 0)
\tjset{weak_d1_rows}{767} % `per_family_test` (rows, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_escalation}{58.0\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s1}{64.8\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d1_s2}{91.7\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 1)
\tjset{weak_d2_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_escalation}{71.7\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s1}{54.7\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d2_s2}{86.5\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 2)
\tjset{weak_d3_rows}{791} % `per_family_test` (rows, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_escalation}{89.8\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s1}{37.3\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d3_s2}{86.3\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 3)
\tjset{weak_d4_rows}{776} % `per_family_test` (rows, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_escalation}{93.4\%} % `per_family_test` (escalation_rate, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s1}{36.6\%} % `per_family_test` (s1_accuracy, row-weighted over owned families at difficulty 4)
\tjset{weak_d4_s2}{85.4\%} % `per_family_test` (s2_accuracy, row-weighted over owned families at difficulty 4)
\tjset{jb_s1_correct}{205} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s1` (correct)
\tjset{jb_s1_acc}{88.7\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s1` (accuracy)
\tjset{jb_s1_hard_correct}{86} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s1` (by_tier.hard.correct)
\tjset{jb_s1_hard_acc}{77.5\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s1` (by_tier.hard.accuracy)
\tjset{jb_s1_ece}{0.037} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s1` (ece)
\tjset{jb_s1_think}{0} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s1` (mean_think_tokens)
\tjset{jb_s1_escalation}{0.0\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s1` (escalation_rate)
\tjset{jb_s1_vs_jev1130_all_ours}{10} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.jev-1.13.0.all` (ours_only)
\tjset{jb_s1_vs_jev1130_all_theirs}{5} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.jev-1.13.0.all` (theirs_only)
\tjset{jb_s1_vs_jev1130_all_p}{$p = 0.302$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.jev-1.13.0.all` (p_value)
\tjset{jb_s1_vs_jev1130_hard_ours}{10} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.jev-1.13.0.hard` (ours_only)
\tjset{jb_s1_vs_jev1130_hard_theirs}{5} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s1_vs_jev1130_hard_p}{$p = 0.302$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.jev-1.13.0.hard` (p_value)
\tjset{jb_s1_vs_openjevthinking_all_ours}{12} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.openjev-thinking.all` (ours_only)
\tjset{jb_s1_vs_openjevthinking_all_theirs}{12} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.openjev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_all_p}{$p = 1.000$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.openjev-thinking.all` (p_value)
\tjset{jb_s1_vs_openjevthinking_hard_ours}{12} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.openjev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_openjevthinking_hard_theirs}{11} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.openjev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_openjevthinking_hard_p}{$p = 1.000$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.openjev-thinking.hard` (p_value)
\tjset{jb_s1_vs_djevthinking_all_ours}{21} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.djev-thinking.all` (ours_only)
\tjset{jb_s1_vs_djevthinking_all_theirs}{18} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.djev-thinking.all` (theirs_only)
\tjset{jb_s1_vs_djevthinking_all_p}{$p = 0.749$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.djev-thinking.all` (p_value)
\tjset{jb_s1_vs_djevthinking_hard_ours}{18} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.djev-thinking.hard` (ours_only)
\tjset{jb_s1_vs_djevthinking_hard_theirs}{17} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.djev-thinking.hard` (theirs_only)
\tjset{jb_s1_vs_djevthinking_hard_p}{$p = 1.000$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.djev-thinking.hard` (p_value)
\tjset{jb_s1_vs_semifqwen354b_all_ours}{24} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_all_theirs}{6} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_all_p}{$p = 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s1_vs_semifqwen354b_hard_ours}{23} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s1_vs_semifqwen354b_hard_theirs}{5} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s1_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s1_vs_reflex27b_all_ours}{6} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.reflex-27b.all` (ours_only)
\tjset{jb_s1_vs_reflex27b_all_theirs}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.reflex-27b.all` (theirs_only)
\tjset{jb_s1_vs_reflex27b_all_p}{$p = 0.289$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.reflex-27b.all` (p_value)
\tjset{jb_s1_vs_reflex27b_hard_ours}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.reflex-27b.hard` (ours_only)
\tjset{jb_s1_vs_reflex27b_hard_theirs}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.reflex-27b.hard` (theirs_only)
\tjset{jb_s1_vs_reflex27b_hard_p}{$p = 0.688$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.reflex-27b.hard` (p_value)
\tjset{jb_s1_vs_deepseekflash_all_ours}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.deepseek-flash.all` (ours_only)
\tjset{jb_s1_vs_deepseekflash_all_theirs}{24} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.deepseek-flash.all` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.deepseek-flash.all` (p_value)
\tjset{jb_s1_vs_deepseekflash_hard_ours}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.deepseek-flash.hard` (ours_only)
\tjset{jb_s1_vs_deepseekflash_hard_theirs}{23} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.deepseek-flash.hard` (theirs_only)
\tjset{jb_s1_vs_deepseekflash_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.deepseek-flash.hard` (p_value)
\tjset{jb_s1_vs_gpt56luna_all_ours}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s1_vs_gpt56luna_all_theirs}{22} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.gpt-5.6-luna.all` (p_value)
\tjset{jb_s1_vs_gpt56luna_hard_ours}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s1_vs_gpt56luna_hard_theirs}{22} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s1_vs_gpt56luna_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s1.gpt-5.6-luna.hard` (p_value)
\tjset{jb_s2_correct}{230} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s2` (correct)
\tjset{jb_s2_acc}{99.6\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s2` (accuracy)
\tjset{jb_s2_hard_correct}{110} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s2` (by_tier.hard.correct)
\tjset{jb_s2_hard_acc}{99.1\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s2` (by_tier.hard.accuracy)
\tjset{jb_s2_ece}{0.091} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s2` (ece)
\tjset{jb_s2_think}{524} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s2` (mean_think_tokens)
\tjset{jb_s2_escalation}{100.0\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.s2` (escalation_rate)
\tjset{jb_s2_vs_jev1130_all_ours}{31} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.jev-1.13.0.all` (ours_only)
\tjset{jb_s2_vs_jev1130_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.jev-1.13.0.all` (theirs_only)
\tjset{jb_s2_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.jev-1.13.0.all` (p_value)
\tjset{jb_s2_vs_jev1130_hard_ours}{30} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.jev-1.13.0.hard` (ours_only)
\tjset{jb_s2_vs_jev1130_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.jev-1.13.0.hard` (theirs_only)
\tjset{jb_s2_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.jev-1.13.0.hard` (p_value)
\tjset{jb_s2_vs_openjevthinking_all_ours}{26} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.openjev-thinking.all` (ours_only)
\tjset{jb_s2_vs_openjevthinking_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.openjev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.openjev-thinking.all` (p_value)
\tjset{jb_s2_vs_openjevthinking_hard_ours}{26} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.openjev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_openjevthinking_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.openjev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_openjevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.openjev-thinking.hard` (p_value)
\tjset{jb_s2_vs_djevthinking_all_ours}{29} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.djev-thinking.all` (ours_only)
\tjset{jb_s2_vs_djevthinking_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.djev-thinking.all` (theirs_only)
\tjset{jb_s2_vs_djevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.djev-thinking.all` (p_value)
\tjset{jb_s2_vs_djevthinking_hard_ours}{26} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.djev-thinking.hard` (ours_only)
\tjset{jb_s2_vs_djevthinking_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.djev-thinking.hard` (theirs_only)
\tjset{jb_s2_vs_djevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.djev-thinking.hard` (p_value)
\tjset{jb_s2_vs_semifqwen354b_all_ours}{43} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_all_theirs}{0} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_s2_vs_semifqwen354b_hard_ours}{42} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_s2_vs_semifqwen354b_hard_theirs}{0} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_s2_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_s2_vs_reflex27b_all_ours}{30} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.reflex-27b.all` (ours_only)
\tjset{jb_s2_vs_reflex27b_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.reflex-27b.all` (theirs_only)
\tjset{jb_s2_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.reflex-27b.all` (p_value)
\tjset{jb_s2_vs_reflex27b_hard_ours}{27} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.reflex-27b.hard` (ours_only)
\tjset{jb_s2_vs_reflex27b_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.reflex-27b.hard` (theirs_only)
\tjset{jb_s2_vs_reflex27b_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.reflex-27b.hard` (p_value)
\tjset{jb_s2_vs_deepseekflash_all_ours}{5} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.deepseek-flash.all` (ours_only)
\tjset{jb_s2_vs_deepseekflash_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.deepseek-flash.all` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_all_p}{$p = 0.219$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.deepseek-flash.all` (p_value)
\tjset{jb_s2_vs_deepseekflash_hard_ours}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.deepseek-flash.hard` (ours_only)
\tjset{jb_s2_vs_deepseekflash_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.deepseek-flash.hard` (theirs_only)
\tjset{jb_s2_vs_deepseekflash_hard_p}{$p = 0.375$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.deepseek-flash.hard` (p_value)
\tjset{jb_s2_vs_gpt56luna_all_ours}{6} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (ours_only)
\tjset{jb_s2_vs_gpt56luna_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_all_p}{$p = 0.125$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.gpt-5.6-luna.all` (p_value)
\tjset{jb_s2_vs_gpt56luna_hard_ours}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_s2_vs_gpt56luna_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_s2_vs_gpt56luna_hard_p}{$p = 0.375$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.s2.gpt-5.6-luna.hard` (p_value)
\tjset{jb_gate_correct}{226} % `jevbench-qwen3.8-27b-report-v2.json` `policies.gate` (correct)
\tjset{jb_gate_acc}{97.8\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.gate` (accuracy)
\tjset{jb_gate_hard_correct}{106} % `jevbench-qwen3.8-27b-report-v2.json` `policies.gate` (by_tier.hard.correct)
\tjset{jb_gate_hard_acc}{95.5\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.gate` (by_tier.hard.accuracy)
\tjset{jb_gate_ece}{0.038} % `jevbench-qwen3.8-27b-report-v2.json` `policies.gate` (ece)
\tjset{jb_gate_think}{264} % `jevbench-qwen3.8-27b-report-v2.json` `policies.gate` (mean_think_tokens)
\tjset{jb_gate_escalation}{24.7\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.gate` (escalation_rate)
\tjset{jb_gate_vs_jev1130_all_ours}{28} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.jev-1.13.0.all` (ours_only)
\tjset{jb_gate_vs_jev1130_all_theirs}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.jev-1.13.0.all` (theirs_only)
\tjset{jb_gate_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.jev-1.13.0.all` (p_value)
\tjset{jb_gate_vs_jev1130_hard_ours}{27} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.jev-1.13.0.hard` (ours_only)
\tjset{jb_gate_vs_jev1130_hard_theirs}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.jev-1.13.0.hard` (theirs_only)
\tjset{jb_gate_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.jev-1.13.0.hard` (p_value)
\tjset{jb_gate_vs_openjevthinking_all_ours}{23} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.openjev-thinking.all` (ours_only)
\tjset{jb_gate_vs_openjevthinking_all_theirs}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.openjev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.openjev-thinking.all` (p_value)
\tjset{jb_gate_vs_openjevthinking_hard_ours}{23} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.openjev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_openjevthinking_hard_theirs}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.openjev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_openjevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.openjev-thinking.hard` (p_value)
\tjset{jb_gate_vs_djevthinking_all_ours}{27} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.djev-thinking.all` (ours_only)
\tjset{jb_gate_vs_djevthinking_all_theirs}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.djev-thinking.all` (theirs_only)
\tjset{jb_gate_vs_djevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.djev-thinking.all` (p_value)
\tjset{jb_gate_vs_djevthinking_hard_ours}{24} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.djev-thinking.hard` (ours_only)
\tjset{jb_gate_vs_djevthinking_hard_theirs}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.djev-thinking.hard` (theirs_only)
\tjset{jb_gate_vs_djevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.djev-thinking.hard` (p_value)
\tjset{jb_gate_vs_semifqwen354b_all_ours}{40} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_gate_vs_semifqwen354b_hard_ours}{39} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_gate_vs_semifqwen354b_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_gate_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_gate_vs_reflex27b_all_ours}{26} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.reflex-27b.all` (ours_only)
\tjset{jb_gate_vs_reflex27b_all_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.reflex-27b.all` (theirs_only)
\tjset{jb_gate_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.reflex-27b.all` (p_value)
\tjset{jb_gate_vs_reflex27b_hard_ours}{23} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.reflex-27b.hard` (ours_only)
\tjset{jb_gate_vs_reflex27b_hard_theirs}{1} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.reflex-27b.hard` (theirs_only)
\tjset{jb_gate_vs_reflex27b_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.reflex-27b.hard` (p_value)
\tjset{jb_gate_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.deepseek-flash.all` (ours_only)
\tjset{jb_gate_vs_deepseekflash_all_theirs}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.deepseek-flash.all` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_all_p}{$p = 1.000$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.deepseek-flash.all` (p_value)
\tjset{jb_gate_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.deepseek-flash.hard` (ours_only)
\tjset{jb_gate_vs_deepseekflash_hard_theirs}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.deepseek-flash.hard` (theirs_only)
\tjset{jb_gate_vs_deepseekflash_hard_p}{$p = 1.000$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.deepseek-flash.hard` (p_value)
\tjset{jb_gate_vs_gpt56luna_all_ours}{5} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (ours_only)
\tjset{jb_gate_vs_gpt56luna_all_theirs}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_all_p}{$p = 1.000$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.gpt-5.6-luna.all` (p_value)
\tjset{jb_gate_vs_gpt56luna_hard_ours}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_gate_vs_gpt56luna_hard_theirs}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_gate_vs_gpt56luna_hard_p}{$p = 1.000$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.gate.gpt-5.6-luna.hard` (p_value)
\tjset{jb_anytime_correct}{223} % `jevbench-qwen3.8-27b-report-v2.json` `policies.anytime` (correct)
\tjset{jb_anytime_acc}{96.5\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.anytime` (accuracy)
\tjset{jb_anytime_hard_correct}{103} % `jevbench-qwen3.8-27b-report-v2.json` `policies.anytime` (by_tier.hard.correct)
\tjset{jb_anytime_hard_acc}{92.8\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.anytime` (by_tier.hard.accuracy)
\tjset{jb_anytime_ece}{0.026} % `jevbench-qwen3.8-27b-report-v2.json` `policies.anytime` (ece)
\tjset{jb_anytime_think}{231} % `jevbench-qwen3.8-27b-report-v2.json` `policies.anytime` (mean_think_tokens)
\tjset{jb_anytime_escalation}{28.1\%} % `jevbench-qwen3.8-27b-report-v2.json` `policies.anytime` (escalation_rate)
\tjset{jb_anytime_vs_jev1130_all_ours}{26} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.jev-1.13.0.all` (ours_only)
\tjset{jb_anytime_vs_jev1130_all_theirs}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.jev-1.13.0.all` (theirs_only)
\tjset{jb_anytime_vs_jev1130_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.jev-1.13.0.all` (p_value)
\tjset{jb_anytime_vs_jev1130_hard_ours}{25} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (ours_only)
\tjset{jb_anytime_vs_jev1130_hard_theirs}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (theirs_only)
\tjset{jb_anytime_vs_jev1130_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.jev-1.13.0.hard` (p_value)
\tjset{jb_anytime_vs_openjevthinking_all_ours}{22} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.openjev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_all_theirs}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.openjev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.openjev-thinking.all` (p_value)
\tjset{jb_anytime_vs_openjevthinking_hard_ours}{22} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.openjev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_openjevthinking_hard_theirs}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.openjev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_openjevthinking_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.openjev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_djevthinking_all_ours}{27} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.djev-thinking.all` (ours_only)
\tjset{jb_anytime_vs_djevthinking_all_theirs}{6} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.djev-thinking.all` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.djev-thinking.all` (p_value)
\tjset{jb_anytime_vs_djevthinking_hard_ours}{24} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.djev-thinking.hard` (ours_only)
\tjset{jb_anytime_vs_djevthinking_hard_theirs}{6} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.djev-thinking.hard` (theirs_only)
\tjset{jb_anytime_vs_djevthinking_hard_p}{$p = 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.djev-thinking.hard` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_all_ours}{39} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_all_theirs}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.all` (p_value)
\tjset{jb_anytime_vs_semifqwen354b_hard_ours}{38} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (ours_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_theirs}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (theirs_only)
\tjset{jb_anytime_vs_semifqwen354b_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.semif-qwen3.5-4b.hard` (p_value)
\tjset{jb_anytime_vs_reflex27b_all_ours}{22} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.reflex-27b.all` (ours_only)
\tjset{jb_anytime_vs_reflex27b_all_theirs}{0} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.reflex-27b.all` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_all_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.reflex-27b.all` (p_value)
\tjset{jb_anytime_vs_reflex27b_hard_ours}{19} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.reflex-27b.hard` (ours_only)
\tjset{jb_anytime_vs_reflex27b_hard_theirs}{0} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.reflex-27b.hard` (theirs_only)
\tjset{jb_anytime_vs_reflex27b_hard_p}{$p < 0.001$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.reflex-27b.hard` (p_value)
\tjset{jb_anytime_vs_deepseekflash_all_ours}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.deepseek-flash.all` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_all_theirs}{7} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.deepseek-flash.all` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_all_p}{$p = 0.549$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.deepseek-flash.all` (p_value)
\tjset{jb_anytime_vs_deepseekflash_hard_ours}{3} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.deepseek-flash.hard` (ours_only)
\tjset{jb_anytime_vs_deepseekflash_hard_theirs}{7} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.deepseek-flash.hard` (theirs_only)
\tjset{jb_anytime_vs_deepseekflash_hard_p}{$p = 0.344$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.deepseek-flash.hard` (p_value)
\tjset{jb_anytime_vs_gpt56luna_all_ours}{4} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_all_theirs}{6} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_all_p}{$p = 0.754$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.all` (p_value)
\tjset{jb_anytime_vs_gpt56luna_hard_ours}{2} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (ours_only)
\tjset{jb_anytime_vs_gpt56luna_hard_theirs}{6} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (theirs_only)
\tjset{jb_anytime_vs_gpt56luna_hard_p}{$p = 0.289$} % `jevbench-qwen3.8-27b-report-v2.json` `paired.anytime.gpt-5.6-luna.hard` (p_value)
\tjset{jb_sys_jev1130_correct}{200} % `jevbench-qwen3.8-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (correct)
\tjset{jb_sys_jev1130_acc}{86.6\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_jev1130_hard_correct}{81} % `jevbench-qwen3.8-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_jev1130_hard_acc}{73.0\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.jev-1.13.0`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_openjevthinking_correct}{205} % `jevbench-qwen3.8-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_openjevthinking_acc}{88.7\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_openjevthinking_hard_correct}{85} % `jevbench-qwen3.8-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_openjevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.openjev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_djevthinking_correct}{202} % `jevbench-qwen3.8-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (correct)
\tjset{jb_sys_djevthinking_acc}{87.4\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_djevthinking_hard_correct}{85} % `jevbench-qwen3.8-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_djevthinking_hard_acc}{76.6\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.djev-thinking`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_semifqwen354b_correct}{187} % `jevbench-qwen3.8-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (correct)
\tjset{jb_sys_semifqwen354b_acc}{81.0\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_semifqwen354b_hard_correct}{68} % `jevbench-qwen3.8-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_semifqwen354b_hard_acc}{61.3\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.semif-qwen3.5-4b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_reflex27b_correct}{201} % `jevbench-qwen3.8-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (correct)
\tjset{jb_sys_reflex27b_acc}{87.0\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_reflex27b_hard_correct}{84} % `jevbench-qwen3.8-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_reflex27b_hard_acc}{75.7\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.reflex-27b`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_deepseekflash_correct}{226} % `jevbench-qwen3.8-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (correct)
\tjset{jb_sys_deepseekflash_acc}{97.8\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_deepseekflash_hard_correct}{107} % `jevbench-qwen3.8-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_deepseekflash_hard_acc}{96.4\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.deepseek-flash`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_sys_gpt56luna_correct}{225} % `jevbench-qwen3.8-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (correct)
\tjset{jb_sys_gpt56luna_acc}{97.4\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (accuracy)
\tjset{jb_sys_gpt56luna_hard_correct}{107} % `jevbench-qwen3.8-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.correct)
\tjset{jb_sys_gpt56luna_hard_acc}{96.4\%} % `jevbench-qwen3.8-27b-report-v2.json` `systems.gpt-5.6-luna`, from JevBench's per-task file (by_tier.hard.accuracy)
\tjset{jb_rows}{231} % `jevbench-qwen3.8-27b-report-v2.json` `policies.*.n`
\tjset{jb_hard_rows}{111} % `jevbench-qwen3.8-27b-report-v2.json` `policies.*.by_tier.hard.n`


==> figures/qwen3.8-27b/per_source.tex <==
A & Escalation (CLINC) & en & -- & 290 & 65.2\% & 80.7\% & 80.7\% & 44.5\% \\
A & Every judgments & en & -- & 84 & 96.4\% & 97.6\% & 97.6\% & 7.1\% \\
A & Intent routing (BANKING77) & en & -- & 486 & 85.6\% & 87.2\% & 87.2\% & 14.2\% \\
A & Intent routing (CLINC) & en & -- & 358 & 95.0\% & 96.9\% & 96.4\% & 8.7\% \\
A & NLI (WANLI) & en & -- & 159 & 74.2\% & 77.4\% & 76.7\% & 24.5\% \\
A & SemIf authored & en & -- & 84 & 94.0\% & 97.6\% & 97.6\% & 13.1\% \\
A & Typed decisions & en & -- & 1165 & 72.8\% & 73.2\% & 74.0\% & 57.9\% \\
\midrule
B & BIG-Bench Hard & en & -- & 620 & 69.5\% & 93.1\% & 92.9\% & 56.5\% \\
B & GPQA Diamond & en & -- & 117 & 48.7\% & 75.2\% & 75.2\% & 83.8\% \\
B & MMLU-Pro & en & -- & 715 & 51.3\% & 78.7\% & 78.3\% & 67.1\% \\
B & MuSR & en & -- & 383 & 59.0\% & 67.9\% & 66.1\% & 43.6\% \\
B & SuperGPQA & en & -- & 652 & 42.0\% & 53.7\% & 54.4\% & 79.0\% \\
\midrule
C & Chess (Lichess) & en & 1 & 121 & 54.5\% & 62.0\% & 64.5\% & 81.0\% \\
C & Chess (Lichess) & en & 2 & 125 & 30.4\% & 41.6\% & 42.4\% & 93.6\% \\
C & Chess (Lichess) & en & 3 & 126 & 29.4\% & 44.4\% & 44.4\% & 96.0\% \\
C & Chess (Lichess) & en & 4 & 122 & 25.4\% & 44.3\% & 44.3\% & 99.2\% \\
C & Chess (Lichess) & zh & 1 & 58 & 53.4\% & 69.0\% & 70.7\% & 87.9\% \\
C & Chess (Lichess) & zh & 2 & 59 & 45.8\% & 47.5\% & 47.5\% & 96.6\% \\
C & Chess (Lichess) & zh & 3 & 60 & 35.0\% & 45.0\% & 45.0\% & 100.0\% \\
C & Chess (Lichess) & zh & 4 & 62 & 27.4\% & 43.5\% & 43.5\% & 100.0\% \\
C & Generated families & en & 1 & 356 & 68.8\% & 100.0\% & 98.3\% & 49.2\% \\
C & Generated families & en & 2 & 362 & 60.2\% & 99.4\% & 93.4\% & 61.9\% \\
C & Generated families & en & 3 & 358 & 38.5\% & 98.9\% & 95.0\% & 86.9\% \\
C & Generated families & en & 4 & 369 & 39.6\% & 98.1\% & 95.1\% & 90.5\% \\
C & Generated families & zh & 1 & 232 & 66.8\% & 100.0\% & 99.1\% & 52.2\% \\
C & Generated families & zh & 2 & 245 & 61.2\% & 99.6\% & 95.5\% & 69.0\% \\
C & Generated families & zh & 3 & 247 & 40.1\% & 99.6\% & 93.9\% & 88.3\% \\
C & Generated families & zh & 4 & 223 & 40.4\% & 98.7\% & 96.9\% & 93.3\% \\
C & hard200 fixture & en & -- & 121 & 80.2\% & 100.0\% & 93.4\% & 40.5\% \\

